Defining an Evaluation Method for External Human-Machine Interfaces

As the number of fatalities involving Autonomous Vehicles increase, the need for a universal method of communicating between vehicles and other agents on the road has also increased. Over the past decade, numerous proposals of external Human-Machine Interfaces (eHMIs) have been brought forward with the purpose of bridging this communication gap, with none yet to be determined as the ideal one. This work proposes a universal evaluation method conformed of 223 questions to objectively evaluate and compare different proposals and arrive at a conclusion. The questionnaire is divided into 7 categories that evaluate different aspects of any given proposal that uses eHMIs: ease of standardization, cost effectiveness, accessibility, ease of understanding, multifacetedness in communication, positioning, and readability. In order to test the method it was used on four existing proposals, plus a baseline using only kinematic motions, in order to both exemplify the application of the evaluation method and offer a baseline score for future comparison. The result of this testing suggests that the ideal method of machine-human communication is a combination of intentionally-designed vehicle kinematics and distributed well-placed text-based displays, but it also reveals knowledge gaps in the readability of eHMIs and the speed at which different observers may learn their meaning. This paper proposes future work related to these uncertainties, along with future testing with the proposed method.

==> image_inserts/FBL_sample.tex <==
\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.75\linewidth]{images/frontalbrakinglights.png}
    \caption{Version of frontal braking lights being evaluated.}
    \label{fig:fbl_example}
\end{figure*}

==> image_inserts/knightrider_sample.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{images/grill_knightrider.png}
    \caption{Example of the Knight Rider display mid-animation.}
    \label{fig:kr_example}
\end{figure}

==> image_inserts/no_eHMI_sample.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{images/baseline.png}
    \caption{The baseline example with no eHMIs.}
    \label{fig:baseline_example}
\end{figure}

==> image_inserts/positioning_configurations.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth,clip,keepaspectratio]{images/Positioning Simulations Graph.png}
    \caption{Diagram illustrating the configurations used to determine visibility. }
    \label{fig:positioning_configurations}
\end{figure*}

==> image_inserts/run_sample.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=4in,clip,keepaspectratio]{images/SUV_RightLane_Front.png}
    \caption{Results showing how many times a Grid Point was recorded, across
all scenarios where the vehicle was an SUV driving North, on the left side of
the virtual environment, and the observer was looking North, towards the front of the vehicle.}
    \label{fig:run_sample}
\end{figure}

==> image_inserts/smile_sample.tex <==
\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.75\linewidth]{images/grill_smile.png}
    \caption{Example of the smiling display, taken from a promotional video of the Smiling Car concept \cite{noauthor_smiling_nodate}.}
    \label{fig:smile_example}
\end{figure*}

==> image_inserts/text_display_sample.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{images/grill_text.png}
    \caption{Example of a text display on the front bumper of a vehicle.}
    \label{fig:text_example}
\end{figure}

==> image_inserts/vehicle_part_diagram.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width={0.8\linewidth},clip,keepaspectratio]{images/Vehicle Diagram.png}
    \caption{Diagram illustrating the external parts of the vehicle as defined by this section of the questionnaire.}
    \label{fig:vehicle_part_diagram}
\end{figure}

==> question_design/light_conditions.tex <==
\paragraph{Light Conditions}
This refers to the lighting conditions of the interaction. The questionnaire scores clear visibility under five difference ranges of lighting conditions, based on the illuminance values of ten light sources and conditions, as recorded by Schlyter \cite{schlyter_radiometry_2023} and the American Meteorological Society \cite{american_metereological_society_civil_2024}:
\begin{itemize}
    \item Between a moonless night with overcasted sky (0.0001 \textit{lx}) and moonless night with airglow (0.002 \textit{lx}) 
    \item Between the dark limit of civil twilight (3.5 \textit{lx}) and a public area with dark surroundings (1000 \textit{lx})
    \item Between a very dark overcast day (100 lx)  and a normal overcast day (1000 \textit{lx}) 
    \item Between full daylight without direct sun (10000 \textit{lx} to 25000 \textit{lx}) and full Daylight with the sun overhead (130000 \textit{lx})
\end{itemize}

==> question_design/weather_conditions.tex <==
\paragraph{Weather Conditions}
These questions focus on the readability of the eHMI under three different levels of rain (as defined by Skilling \cite{skilling_meteorologists_2018}), three different levels of fog (as defined by the U.S. Department of Commerce \cite{us_department_of_commerce_about_nodate}), and when lighting is present. 

==> questionnaires/qa.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
%\begin{table*}[ht]
\caption{Accessibility Questionnaire}
\label{tab:QA_table}
\begin{tabular}{|p{0.5cm} | p{0.5cm} | p{15.2cm}|}
\hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{3}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{ACCESSIBILITY}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{ID}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{PTS}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{QUESTION}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{GENERAL} \\ \hline
\multicolumn{1}{|c|}{A1} & \multicolumn{1}{c|}{1} & All visible eHMI in this proposal use pictograms. \\ \hline
\multicolumn{1}{|c|}{A2} & \multicolumn{1}{c|}{1} & All visible eHMI in this proposal use text. \\ \hline
\multicolumn{1}{|c|}{A3} & \multicolumn{1}{c|}{1} & This proposal includes a tactile component. \\ \hline
\multicolumn{1}{|c|}{A4} & \multicolumn{1}{c|}{1} & This proposal includes sound cues. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{VISUAL - GENERAL} \\ \hline
\multicolumn{1}{|c|}{A5} & \multicolumn{1}{c|}{1} & The placement of information is not affected by vehicle type or size. \\ \hline
\multicolumn{1}{|c|}{A6} & \multicolumn{1}{c|}{1} & All information is placed in an isolated space with little visual clutter. \\ \hline
\multicolumn{1}{|c|}{A7} & \multicolumn{1}{c|}{1} & All information is consistently displayed in the same location. \\ \hline
\multicolumn{1}{|c|}{A8} & \multicolumn{1}{c|}{1} & Measures are taken to prevent the creation of shadows on or caused by the information. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}VISUAL - PICTOGRAMS\\ If answered "No" to A1, answer A9 through A14 with “0”\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{A9} & \multicolumn{1}{c|}{1} & All pictograms contrast with their surroundings. \\ \hline
\multicolumn{1}{|c|}{A10} & \multicolumn{1}{c|}{1} & All pictograms are always upright. \\ \hline
\multicolumn{1}{|c|}{A11} & \multicolumn{1}{c|}{1} & All pictograms use bold, uniform, thick lines. \\ \hline
\multicolumn{1}{|c|}{A12} & \multicolumn{1}{c|}{1} & All pictograms use straight lines. \\ \hline
\multicolumn{1}{|c|}{A13} & \multicolumn{1}{c|}{1} & All pictograms are fully distinct from each other with no shared elements. \\ \hline
\multicolumn{1}{|c|}{A14} & \multicolumn{1}{c|}{1} & All pictograms and their backgrounds are non-reflective and anti-glare. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}VISUAL - BACKGROUND\\ If answered "No" to A1 and A2, answer A15 through A17 with “0”\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{A15} & \multicolumn{1}{c|}{1} & All eHMI(s) in this proposal use a single color background. \\ \hline
\multicolumn{1}{|c|}{A16} & \multicolumn{1}{c|}{1} & All eHMI(s) in this proposal use dark text in a light background. \\ \hline
\multicolumn{1}{|c|}{A17} & \multicolumn{1}{c|}{1} & All eHMI(s) in this proposal avoid pure-white bright white background. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}VISUAL - TEXT\\ If answered "No" to A2, answer A18 through A29 with “0”\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{A18} & \multicolumn{1}{c|}{1} & All text contrasts with its surroundings. \\ \hline
\multicolumn{1}{|c|}{A19} & \multicolumn{1}{c|}{1} & All text is straight and readable. \\ \hline
\multicolumn{1}{|c|}{A20} & \multicolumn{1}{c|}{1} & None of the text is in italics. \\ \hline
\multicolumn{1}{|c|}{A21} & \multicolumn{1}{c|}{1} & All text uses bold, uniform, thick lines. \\ \hline
\multicolumn{1}{|c|}{A22} & \multicolumn{1}{c|}{1} & All text uses straight lines. \\ \hline
\multicolumn{1}{|c|}{A23} & \multicolumn{1}{c|}{1} & All text characters are distinct from each other. \\ \hline
\multicolumn{1}{|c|}{A24} & \multicolumn{1}{c|}{1} & All text characters include prominent ascenders, descenders, and open counterforms. \\ \hline
\multicolumn{1}{|c|}{A25} & \multicolumn{1}{c|}{1} & All text and its background are non-reflective (No glare). \\ \hline
\multicolumn{1}{|c|}{A26} & \multicolumn{1}{c|}{1} & All text uses initial uppercase letters and is not in all caps. \\ \hline
\multicolumn{1}{|c|}{A27} & \multicolumn{1}{c|}{1} & All text fonts and typefaces have wide horizontal proportions. \\ \hline
\multicolumn{1}{|c|}{A28} & \multicolumn{1}{c|}{1} & The text does not rotate. \\ \hline
\multicolumn{1}{|c|}{A29} & \multicolumn{1}{c|}{1} & The text does not include hyphens (-) and em dashes (—). \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}VISUAL - COLOR\\ If non applicable, answer A30 and A34 with "1"\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{A30} & \multicolumn{1}{c|}{1} & The eHMI(s) in this proposal do not depend exclusively on color to communicate any information. \\ \hline
\multicolumn{1}{|c|}{A31} & \multicolumn{1}{c|}{1} & The proposal avoids combinations of colors most commonly confused by color blind people, such as red, green, brown, and orange. \\ \hline
\multicolumn{1}{|c|}{A32} & \multicolumn{1}{c|}{$\frac{Cu}{Cuu}$} & \begin{tabular}[c]{@{}l@{}}COLOR ASSOCIATION \\ (Cuu: Number of colors used by this eHMI - such as cyan, blue-green, and turquoise - that do not have a previous association in\\ the road.\\ Cu: Total number of colors used by this eHMI)\\ If this proposal does not use color, answer with a 1.\end{tabular} \\ \hline
\multicolumn{1}{|c|}{A33} & \multicolumn{1}{c|}{1} & The color(s) used by the visual eHMIs in this proposal can be adjusted during manufacturing or shipping to adjust to local regulation. \\ \hline
\multicolumn{1}{|c|}{A34} & \multicolumn{1}{c|}{1} & The proposal includes in it a color or design for the eHMI(s) so that it will not blend in with the rest of the vehicle, regardless of its paint job. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}TACTILE\\ If answered "No" to A3, answer A35 with “0”\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{A35} & \multicolumn{1}{c|}{1} & This proposal has a tactile component without employing braille, or it uses braille with signage standardization (shape, size, distance, etc). \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}AUDITORY\\ If answered "No" to A4, answer A36 through A41 with “0”\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{A36} & \multicolumn{1}{c|}{1} & The speakers in this proposal use speakers that minimize echo. \\ \hline
\multicolumn{1}{|c|}{A37} & \multicolumn{1}{c|}{1} & All sound cues in this proposal are distinguishable from other road sounds. \\ \hline
\multicolumn{1}{|c|}{A38} & \multicolumn{1}{c|}{1} & All sound cues in this proposal are clearly distinguishable from each other. \\ \hline
\multicolumn{1}{|c|}{A39} & \multicolumn{1}{c|}{1} & All non-verbal signals have a maximum frequency of 1500 Hz \\ \hline
\multicolumn{1}{|c|}{A40} & \multicolumn{1}{c|}{1} & All audible verbal signals have a frequency between 300 Hz and 3000 Hz \\ \hline
\multicolumn{1}{|c|}{A41} & \multicolumn{1}{c|}{1} & All sounds have a volume of between 10 dB and 80 dB, above ambient. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{NEUROLOGICAL} \\ \hline
\multicolumn{1}{|c|}{A42} & \multicolumn{1}{c|}{1} & None of the visual eHMI(s) in this proposal use flashing lights. \\ \hline
\multicolumn{1}{|c|}{A43} & \multicolumn{1}{c|}{1} & None of the visual eHMI(s) in this proposal contain any elements that flash more than three times in any one second. \\ \hline
\multicolumn{1}{|c|}{A44} & \multicolumn{1}{c|}{1} & None of the visual eHMI(s) in this proposal use the color red. \\ \hline
\multicolumn{1}{|c|}{A45} & \multicolumn{1}{c|}{1} & None of the visual eHMI(s) in this proposal use animations, or all animations employed are simple moving elements. \\ \hline
\multicolumn{1}{|c|}{A46} & \multicolumn{1}{c|}{1} & None of the visual eHMI(s) in this proposal use animations with parallax. \\ \hline
\end{tabular}
%\end{table*}

%\input{questionnaires/qa2}

==> questionnaires/qa2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
%\begin{table*}[ht]
%\label{tab:QA_table}
%\caption{part 2}
\begin{tabular}{|p{0.5cm} | p{0.5cm} | p{15.2cm}|}
\hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{COGNITIVE - GENERAL} \\ \hline
A47 & 1 & This proposal uses text, all of which is short and concise. \\ \hline
A48 & 1 & All information provides enough time to be read and understood comfortably by the average pedestrian or driver. \\ \hline
A49 & 1 & All information is presented in more than one way at a time. \\ \hline
A50 & 1 & The eHMI(s) in this proposal presents information explicitly and directly to the observer (e.g. symbol aimed at pedestrians shows a person walking, instead of an arrow). \\ \hline
A51 & 1 & The eHMI(s) in this proposal present information in an egocentric approach to communicate information (i.e. “Walk” instead of “Stopping” when yielding). Score with 0 if not applicable. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{COGNITIVE - LANGUAGE} \\ \hline
A52 & 1 & The eHMI(s) in this proposal don't use text, or use text with plain language. \\ \hline
A53 & 1 & The eHMI(s) in this proposal don't use text or use text without making use of idioms (phrases whose meaning cannot be deduced from the meaning of the individual words). \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}p{15.2cm}@{}}COGNITIVE - CULTURAL\\ Rounding up, what percentage of the non-textual components (pictograms, lights, sounds, tactile components, etc) of the \\total eHMI(s) in this proposal are not universal, and hence may hold different meanings depending on local factors \\(e.g. language, culture)? If not applicable, score A54 through A58 with 1\end{tabular}} \\ \hline
A54 & 1 & 80\% or less \\ \hline
A55 & 1 & 60\% or less \\ \hline
A56 & 1 & 40\% or less \\ \hline
A57 & 1 & 20\% or less \\ \hline
A58 & 1 & 0\%. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}p{15.2cm}@{}}COGNITIVE - CONTEXTUAL\\ Rounding up, what percentage of the non-textual components (pictograms, lights, sounds, tactile components, etc) of the \\total eHMI(s) in this proposal may hold different meanings depending on environmental factors (e.g. weather, time of day,\\ etc)? \\If not applicable, score A59 through A63 with "1"\end{tabular}} \\ \hline
A59 & 1 & 80\% or less \\ \hline
A60 & 1 & 60\% or less \\ \hline
A61 & 1 & 40\% or less \\ \hline
A62 & 1 & 20\% or less \\ \hline
A63 & 1 & 0\%. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}p{15.2cm}@{}}PSYCHOLOGY - DISTRESSING IMAGERY\\ Rounding up, what percentage of all symbols, text, sounds, and tactile components used by the eHMI(s) in this proposal \\could trigger adverse psychological reactions, such as depicting those in distress or feelings of hopelessness? \\If not applicable, score A64 through A68 with "1"\end{tabular}} \\ \hline
A64 & 1 & 80\% or less \\ \hline
A65 & 1 & 60\% or less \\ \hline
A66 & 1 & 40\% or less \\ \hline
A67 & 1 & 20\% or less \\ \hline
A68 & 1 & 0\%. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}p{15.2cm}@{}}PSYCHOLOGY - LANGUAGE\\ Rounding up, what percentage of all symbols, text, sounds, and tactile components used by the eHMI(s) in this proposal \\depict or use language that can be deemed offensive to those within the mental health community, such as “insane”, \\“crazy”, “maniac”, “normal”, etc. If not applicable, score A69 through A73 with "1"\end{tabular}} \\ \hline
A69 & 1 & 80\% or less \\ \hline
A70 & 1 & 60\% or less \\ \hline
A71 & 1 & 40\% or less \\ \hline
A72 & 1 & 20\% or less \\ \hline
A73 & 1 & 0\%. \\ \hline
\end{tabular}
%\end{table*}

==> questionnaires/qc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
%\begin{table*}[ht]
\caption{Color Questionnaire}
\label{tab:QC_table}
\begin{tabular}{|p{0.5cm} | p{0.5cm} | p{15.2cm}|}
\hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{3}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{COLOR}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{ID}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{PTS}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{QUESTION}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{COLOR CHOICE} \\ \hline
\multicolumn{1}{|c|}{C1} & \multicolumn{1}{c|}{1} & In the proposal, at least 1/3 of the when time a visual eHMI is displaying information, said information uses a color without a previous association in the road (cyan, blue-green, turquoise). \\ \hline
\multicolumn{1}{|c|}{C2} & \multicolumn{1}{c|}{1} & In the proposal, at least 2/3 of the when time a visual eHMI is displaying information, said information uses a color without a previous association in the road (cyan, blue-green, turquoise). \\ \hline
\multicolumn{1}{|c|}{C3} & \multicolumn{1}{c|}{1} & In the proposal, visual eHMIs always displays information using a color without a previous association in the road (cyan, blue-green, turquoise). \\ \hline
\multicolumn{1}{|c|}{C4} & \multicolumn{1}{c|}{1} & The color(s) used by the visual eHMIs in this proposal can be adjusted during manufacturing or shipping to adjust to local federal regulation. \\ \hline
\multicolumn{1}{|c|}{C5} & \multicolumn{1}{c|}{1} & The proposal includes in it a color for the eHMI(s) so that it will not blend in with the rest of the vehicle, regardless of its paint job. \\ \hline
\end{tabular}
%\end{table*}

==> questionnaires/qcc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
%\begin{table*}[ht]
\caption{Constant Communication Questionnaire}
\label{tab:QCC_table}
\begin{tabular}{|p{0.5cm} | p{0.5cm} | p{15.2cm}|}
\hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{3}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{CONSTANT COMMUNICATION}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{ID}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{PTS}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{QUESTION}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}ONE-WAY GENERAL COMMUNICATION\\ The eHMI(s) in this proposal can explicitly communicate to observers...\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{CC1} & \multicolumn{1}{c|}{1} & ...when the vehicle is moving forward. \\ \hline
\multicolumn{1}{|c|}{CC2} & \multicolumn{1}{c|}{1} & ...when the vehicle is backing up. \\ \hline
\multicolumn{1}{|c|}{CC3} & \multicolumn{1}{c|}{1} & ...when the vehicle is slowing down. \\ \hline
\multicolumn{1}{|c|}{CC4} & \multicolumn{1}{c|}{1} & ...when the vehicle is speeding up. \\ \hline
\multicolumn{1}{|c|}{CC5} & \multicolumn{1}{c|}{1} & ...when autonomous mode is engaged. \\ \hline
\multicolumn{1}{|c|}{CC6} & \multicolumn{1}{c|}{1} & ...when autonomous mode is not engaged. \\ \hline
\multicolumn{1}{|c|}{CC7} & \multicolumn{1}{c|}{1} & ...when the vehicle is unable to move. \\ \hline
\multicolumn{1}{|c|}{CC8} & \multicolumn{1}{c|}{1} & ...when a door is opening. \\ \hline
\multicolumn{1}{|c|}{CC9} & \multicolumn{1}{c|}{1} & ...when a door is opening, and it specifies which door(s) are opening. \\ \hline
\multicolumn{1}{|c|}{CC10} & \multicolumn{1}{c|}{1} & ...when this vehicle is obscuring another moving vehicle. \\ \hline
\multicolumn{1}{|c|}{CC11} & \multicolumn{1}{c|}{1} & ...when the vehicle is turning, and what direction it's turning to (does not replace blinkers). \\ \hline
\multicolumn{1}{|c|}{CC12} & \multicolumn{1}{c|}{1} & ...when the vehicle is changing lanes, and what lane it's changing into (does not replace blinkers). \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}ONE-WAY PEDESTRIAN COMMUNICATION\\ The eHMI(s) in this proposal can explicitly communicate to pedestrians...\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{CC13} & \multicolumn{1}{c|}{1} & ...when they’ve been detected. \\ \hline
\multicolumn{1}{|c|}{CC14} & \multicolumn{1}{c|}{1} & ...when the vehicle is yielding to them. \\ \hline
\multicolumn{1}{|c|}{CC15} & \multicolumn{1}{c|}{1} & ...when the vehicle is not yielding to them. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}TWO-WAY PEDESTRIAN COMMUNICATION\\ The eHMI(s) in this proposal can explicitly communicate to pedestrians...\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{CC16} & \multicolumn{1}{c|}{1} & ...where the vehicle estimates they are. \\ \hline
\multicolumn{1}{|c|}{CC17} & \multicolumn{1}{c|}{1} & ...how to request the vehicle to be stopped, if applicable. Otherwise, score with 1. \\ \hline
\multicolumn{1}{|c|}{CC18} & \multicolumn{1}{c|}{1} & ...whether the pedestrian's reaction to the vehicle have been detected and interpreted, if applicable. Otherwise, score with 1. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}MALFUNCTIONS\\ The eHMI(s) in this proposal can explicitly communicate externally...\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{CC19} & \multicolumn{1}{c|}{1} & ...when the vehicle estimates it will not be able to prevent an impact. \\ \hline
\multicolumn{1}{|c|}{CC20} & \multicolumn{1}{c|}{1} & ...when the vehicle’s sensors are malfunctioning. \\ \hline
\multicolumn{1}{|c|}{CC21} & \multicolumn{1}{c|}{1} & ...when the vehicle’s driving systems are malfunctioning. \\ \hline
\multicolumn{1}{|c|}{CC22} & \multicolumn{1}{c|}{1} & ...when weather conditions are interfering with the vehicle's driving systems \\ \hline
\multicolumn{1}{|c|}{CC23} & \multicolumn{1}{c|}{1} & ...when weather conditions are interfering with the sensors. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}OTHER\\ The eHMI(s) in this proposal can explicitly communicate externally...\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{CC24} & \multicolumn{1}{c|}{1} & ...when the vehicle is turned on and when it is turned off. \\ \hline
\end{tabular}
%\end{table*}

==> questionnaires/qce.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
%\begin{table*}[ht]
\caption{Cost Effectiveness Questionnaire}
\label{tab:QCE_table}
\centering
%\begin{tabular}{ccl}
\begin{tabular}{|p{0.5cm} | p{0.5cm} | p{15.2cm}|}
\hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{3}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{COST EFFECTIVENESS}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{ID}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{PTS}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{QUESTION}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{All costs should be adjusted for inflation for 2022}} \\ \hline
\multicolumn{1}{|c|}{CE1} & \multicolumn{1}{c|}{Man} & MANUFACTURING COST (Man: The average cost of manufacturing a single set of this technology, without accounting for product development or infrastructure.) \\ \hline
\multicolumn{1}{|c|}{CE2} & \multicolumn{1}{c|}{InsN} & COST OF INSTALLATION ON NEW VEHICLE (ImpN: The average cost of implementing this technology in a new vehicle.) \\ \hline
\multicolumn{1}{|c|}{CE3} & \multicolumn{1}{c|}{InsE} & COST OF INSTALLATION ON EXISTING VEHICLE (ImpE: The average cost of implementing this technology in an existing, operating vehicle.) \\ \hline
\multicolumn{1}{|c|}{CE4} & \multicolumn{1}{c|}{Mai} & MAINTENANCE COST (Mai: The average yearly cost of maintaining this technology once installed.) \\ \hline
\multicolumn{1}{|c|}{CE5} & \multicolumn{1}{c|}{OC} & OPERATION COST (OC: Without accounting for maintenance and replacements, but accounting for any resource consumption such as energy and gasoline, the average yearly cost of operating this technology as intended in a single vehicle.) \\ \hline
\end{tabular}
%\end{table*}

==> questionnaires/qef.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
%\begin{table*}[ht]
\caption{Environmental Sustainability Questionnaire}
\label{tab:QES_table}
\begin{tabular}{|p{0.5cm} | p{0.5cm} | p{15.2cm}|}
\hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{3}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{ENVIRONMENTAL SUSTAINABILITY}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{ID}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{PTS}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{QUESTION}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{LIGHT POLLUTION} \\ \hline
\multicolumn{1}{|c|}{ES1} & \multicolumn{1}{c|}{1} & The eHMI(s) in this proposal are turned off when not in use. \\ \hline
\multicolumn{1}{|c|}{ES2} & \multicolumn{1}{c|}{1} & The eHMI(s) in this proposal do not use lights, or all light fittings are located, directed, or shielded to avoid lighting anything but the target object or area. \\ \hline
\multicolumn{1}{|c|}{ES3} & \multicolumn{1}{c|}{1} & The eHMI(s) in this proposal do not use lights, or they are (all) located close to the ground to reduce sky glow. \\ \hline
\multicolumn{1}{|c|}{ES4} & \multicolumn{1}{c|}{1} & The eHMI(s) in this proposal do not use lights, or light is prevented from shining above the horizontal plane by mounting the luminaire horizontally relative to the ground and not at an angle. \\ \hline
\multicolumn{1}{|c|}{ES5} & \multicolumn{1}{c|}{1} & The eHMI(s) in this proposal do not use lights, or only the minimum number and intensity of light needed to be effective. \\ \hline
\multicolumn{1}{|c|}{ES6} & \multicolumn{1}{c|}{1} & The eHMI(s) in this proposal do not use lights, or use low glare lighting. \\ \hline
\multicolumn{1}{|c|}{ES7} & \multicolumn{1}{c|}{1} & Surfaces on the eHMIs on this proposal that are not part of its communication methods are dark and non-reflective. \\ \hline
\multicolumn{1}{|c|}{ES8} & \multicolumn{1}{c|}{1} & The eHMI(s) in this proposal do not use lights, or their lights have blue wavelengths filtered out. \\ \hline
\multicolumn{1}{|c|}{ES9} & \multicolumn{1}{c|}{1} & The eHMI(s) in this proposal do not use lights, or their lights have violet wavelengths filtered out. \\ \hline
\multicolumn{1}{|c|}{ES10} & \multicolumn{1}{c|}{1} & The eHMI(s) in this proposal do not use lights, or their lights have ultraviolet wavelengths filtered out. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{NOISE POLLUTION} \\ \hline
\multicolumn{1}{|c|}{ES11} & \multicolumn{1}{c|}{2.5} & The eHMI(s) in this proposal do not use sound, or over a period of 24 hours, a sedan passenger vehicle making use of the eHMI(s) in this proposal will not produce noise exceeding 70 decibels on average. \\ \hline
\multicolumn{1}{|c|}{ES12} & \multicolumn{1}{c|}{2.5} & The eHMI(s) in this proposal do not use sound, or over a period of 1 hour, a sedan passenger vehicle making use of the eHMI(s) in this proposal will not produce exceeding 85 decibels on average. \\ \hline
\multicolumn{1}{|c|}{ES13} & \multicolumn{1}{c|}{2.5} & The eHMI(s) in this proposal do not use sounds, or none of the sounds employed by it may possibly confuse, misguide, or negatively affect local wildlife. \\ \hline
\multicolumn{1}{|c|}{ES14} & \multicolumn{1}{c|}{2.5} & The eHMI(s) in this proposal do not use sounds, or none of the sounds employed by it may confuse, misguide, or negatively affect pedestrians or drivers. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{AIR POLLUTION} \\ \hline
\multicolumn{1}{|c|}{ES15} & \multicolumn{1}{c|}{10} & The proposed technolgy does not release any components into the air as part of its intended behavior. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{LAND AND WATER POLLUTION} \\ \hline
\multicolumn{1}{|c|}{ES16} & \multicolumn{1}{c|}{10} & The proposed technolgy does not release any solid components as part of its intended behavior. \\ \hline
\multicolumn{1}{|c|}{ES17} & \multicolumn{1}{c|}{10} & The proposed technolgy does not release any liquid components as part of its intended behavior. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{THERMAL POLLUTION} \\ \hline
\multicolumn{1}{|c|}{ES18} & \multicolumn{1}{c|}{10} & The proposed technolgy does not produce significant heat as part of its intended behavior. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{RADIATION POLLUTION} \\ \hline
\multicolumn{1}{|c|}{ES19} & \multicolumn{1}{c|}{10} & Over a period of 24 hours, a busy road with vehicles making use of this eHMI(s) in this proposal will not expose pedestrians or drivers to more than 1.7 millirem (620 millirem a year). \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{EMISSION PENALTY} \\ \hline
\multicolumn{1}{|c|}{ES20} & \multicolumn{1}{c|}{Ep} & Ep: The total kilogram amount of greenhouse gases produced in a year, directly or indirectly, by all eHMIs in this proposal. \\ \hline
\end{tabular}
%\end{table*}

==> questionnaires/qeu.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
%\begin{table*}[]
\caption{Ease of Understanding Questionnaire}
\label{tab:QEU_table}
\begin{tabular}{|p{0.5cm} | p{0.5cm} | p{15.2cm}|}
\hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{3}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{EASE OF UNDERSTANDING}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{ID}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{PTS}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{QUESTION}} \\ \hline
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}} & \textbf{PEDESTRIANS} \\ \hline
\multicolumn{1}{|c|}{EU1} & \multicolumn{1}{c|}{Mpp} & CLARITY FOR MINOR PEDESTRIANS (Mpp: The "feel-safe percentage" for pedestrians under the age of 18 interacting with this proposal, after nine (9) encounters with a vehicle making use of it.) \\ \hline
\multicolumn{1}{|c|}{EU2} & \multicolumn{1}{c|}{App} & CLARITY FOR ADULT PEDESTRIANS (App:  The "feel-safe percentage" for pedestrians between the age of 18 and 64 interacting with this proposal, after nine (9) encounters with a vehicle making use of it.) \\ \hline
\multicolumn{1}{|c|}{EU3} & \multicolumn{1}{c|}{Epp} & CLARITY FOR ELDERLY PEDESTRIANS (Epp:  The "feel-safe percentage" for pedestrians over the age of 64 interacting with this proposal, after nine (9) encounters with a vehicle making use of it.) \\ \hline
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}} & \textbf{CICLYSTS} \\ \hline
\multicolumn{1}{|c|}{EU4} & \multicolumn{1}{c|}{Mpc} & CLARITY FOR MINOR CYCLISTS (Mpc: The "feel-safe percentage" for cyclists under the age of 18 interacting with this proposal, after nine (9) encounters with a vehicle making use of it.) \\ \hline
\multicolumn{1}{|c|}{EU5} & \multicolumn{1}{c|}{Apc} & CLARITY FOR ADULT CYCLISTS (Apc:  The "feel-safe percentage" for cyclists between the age of 18 and 64 interacting with this proposal, after nine (9) encounters with a vehicle making use of it.) \\ \hline
\multicolumn{1}{|c|}{EU6} & \multicolumn{1}{c|}{Epc} & CLARITY FOR ELDERLY CYCLISTS (Epc:  The "feel-safe percentage" for cyclists over the age of 64 interacting with this proposal, after nine (9) encounters with a vehicle making use of it.) \\ \hline
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}} & \textbf{DRIVERS} \\ \hline
\multicolumn{1}{|c|}{EU7} & \multicolumn{1}{c|}{Ap} & CLARITY FOR ADULT DRIVERS (Ap:  The "feel-safe percentage" for pedestrians between the age of 18 and 64 interacting with this proposal, after nine (9) encounters with a vehicle making use of it.) \\ \hline
\multicolumn{1}{|c|}{EU8} & \multicolumn{1}{c|}{Ep} & CLARITY FOR ELDERLY DRIVERS (Ep:  The "feel-safe percentage" for pedestrians over the age of 64 interacting with this proposal, after nine (9) encounters with a vehicle making use of it.) \\ \hline
\end{tabular}
%\end{table*}

==> questionnaires/qp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
%\begin{table*}[]
\caption{Positioning Questionnaire}
\label{tab:QP_table}
\begin{tabular}{|p{0.5cm} | p{7.5cm} | p{8.5cm}|}
\hline
\rowcolor[HTML]{D9D9D9} 
\textbf{POSITIONING} & \textbf{} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\textbf{ID} & \textbf{PTS} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{QUESTION}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}} & \textbf{MIRRORING AND SYMMETRY} \\ \hline
P1 & 1 & This eHMI is symmetrical accross the length of this vehicle (i.e. the left and right side of the vehicle are symmetrical). \\ \hline
P2 & 2 & This eHMI is standing on the roof of the vehicle. \\ \hline
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}} & \textbf{\begin{tabular}[c]{@{}l@{}}VISIBILITY\\ In a given vehicle, the eHMI can be found on...\end{tabular}} \\ \hline
P3 & P1 + 1 & ...anywhere on the back bumper. \\ \hline
P4 & 2 & ...the back central light. \\ \hline
P5 & P1 + 1 & ...either of the back fenders. \\ \hline
P6 & P1 + 1 & ...anywhere on the back low reflector. \\ \hline
P7 & 2 & ...the location of the back plate. \\ \hline
P8 & P1 + 1 & ...either of the back window rails. \\ \hline
P9 & P1 + 1 & ...anywhere on the back window. \\ \hline
P10 & P1 + 1 & ...anywhere on the back window lower frame. \\ \hline
P11 & 0 & ...anywhere on the cowl cover. \\ \hline
P12 & P1 + 1 & ...anywhere on the front bumper. \\ \hline
P13 & P1 + 1 & ...anywhere on the front low reflector. \\ \hline
P14 & P1 + 1 & ...anywhere on either of the front doors. \\ \hline
P15 & P1 + 1 & ...either of the front fenders. \\ \hline
P16 & 2 & ...the location of the front plate. \\ \hline
P17 & P1 + 1 & ...either of the windshield side rails. \\ \hline
P18 & P1 + 1 & ...either of the front wheels. \\ \hline
P19 & P1 + 1 & ...either of the front windows. \\ \hline
P20 & P1 + 1 & ...anywhere on the grill. \\ \hline
P21 & P1 + 1 & ...either headlight or their surroundings. \\ \hline
P22 & P1 + 1 & ...anywhere on the hood. \\ \hline
P23 & 0 & ...either of the rear doors. \\ \hline
P24 & P1 + 1 & ...either of the rear wheels. \\ \hline
P25 & P1 + 1 & ...either of the back windows. \\ \hline
P26 & P1 + 1 & ...either of the rocker panels. \\ \hline
P27 & P2 & ...roof. \\ \hline
P28 & P1 + 1 & ...either of the side mirrors. \\ \hline
P29 & P1 + 1 & ...either of the side mirror's front. \\ \hline
P30 & P1 + 1 & ...anywhere on the windshield. \\ \hline
P31 & P1 + 1 & ...either tail light. \\ \hline
P32 & P1 + 1 & ...anywhere on the trunk. \\ \hline
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}} & \textbf{\begin{tabular}[c]{@{}l@{}}EHMI(S) PURPOSE\\ The purpose of this eHMI in this proposal is to...\end{tabular}} \\ \hline
P33 & \begin{tabular}[c]{@{}c@{}}$\frac{MAX(P12, P13, P15, P17, P18, P20, P21, P22, P24, P25, P29, P30)}{4}$\\$+\frac{ MAX(P5, P8, P12, P14, P15, P17, P18, P19, P20, P21, P22)}{4}$\end{tabular} & ...inform pedestrians on the sidewalk of the intent of the AV as an approaching vehicle on the road. \\ \hline
P34 & \begin{tabular}[c]{@{}c@{}}$\frac{MAX(P3, P4, P5, P7, P8, P9, P10, P18, P28, P29, P31, P32)}{4}$\\+$\frac{MAX(P15, P21, P22)}{4}$\end{tabular} & ...inform pedestrians on the sidewalk of the intent of the vehicle as it is moving away from them on the road. \\ \hline
P35 & $\frac{MAX(P12, P13, P15, P16, P17, P20, P21, P22, P29, P30)}{2}$ & ...inform pedestrians on the sidewalk as the vehicle comes out of an alleyway or exit that is on the opposite side of the road \\ \hline
P36 & $\frac{MAX(P14, P15, P17, P18, P26)}{2}$ & ...inform pedestrians on the sidewalk of the vehicle's intent as it exits an alleyway or exit that goes over the sidewalk the pedestrian is on. \\ \hline
P37 & $\frac{MAX(P5, P8, P14, P17)}{2}$ & ...inform drivers driving in the opposite direction of the vehicle of its intent. \\ \hline
P38 & $\frac{MAX(P12, P13, P15, P16, P20, P21, P22)}{2}$ & ...inform drivers in front of the vehicle that are driving in the same direction. \\ \hline
P39 & $\frac{MAX(P3, P6, P7, P9, P10, P32)}{2}$ & ...inform drivers behind the vehicle that are driving in the same direction. \\ \hline
P40 & $\frac{MAX(P12, P13, P15, P20, P21, P22)}{2}$ & ...inform drivers on the road as the vehicle is about to turn into it from an alleyway or exit \\ \hline
\end{tabular}
%\end{table*}

==> questionnaires/qr.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
%\begin{table*}[ht]
\caption{Readability Questionnaire}
\label{tab:QR_table}
\begin{tabular}{|p{0.5cm} | p{0.5cm} | p{15.2cm}|}
\hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{3}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{READABILITY}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{ID}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{PTS}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{QUESTION}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{DYNAMIC LIGHT ADAPTATION} \\ \hline
\multicolumn{1}{|c|}{R1} & \multicolumn{1}{c|}{1} & At least 1/3 of the eHMIs described in the proposal can adjust their brightness based on weather and lighting conditions. \\ \hline
\multicolumn{1}{|c|}{R2} & \multicolumn{1}{c|}{1} & At least 2/3 of the eHMIs described in the proposal can adjust their brightness based on weather and lighting conditions. \\ \hline
\multicolumn{1}{|c|}{R3} & \multicolumn{1}{c|}{1} & All of the eHMIs described in the proposal can adjust their brightness based on weather and lighting conditions. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}READABILITY CONDITIONS - LIGHT\\ Accounting for dynamic adjustments if applicable, in clear weather, all relevant eHMI(s) in this proposal 33 feet away \\from the observer are...\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{R4} & \multicolumn{1}{c|}{1} & ...fully readable when placed under an average illuminance of between 0.0001 lux (e.g. moonless night with overcasted sky) and 0.002 lux (e.g. moonless night with airglow). \\ \hline
\multicolumn{1}{|c|}{R5} & \multicolumn{1}{c|}{1} & ...somewhat distinguishable when placed under an average illuminance of between 0.0001 lux (e.g. moonless night with overcasted sky) and 0.002 lux (e.g. moonless night with airglow). Answer 1 if R1 is 1. \\ \hline
\multicolumn{1}{|c|}{R6} & \multicolumn{1}{c|}{1} & ...fully distinguishable when placed under an average illuminance of between 3.5 lux (e.g. dark limit of civil twilight) and 20 lux (e.g. public area with dark surroundings). \\ \hline
\multicolumn{1}{|c|}{R7} & \multicolumn{1}{c|}{1} & ...somewhat distinguishable when placed under an average illuminance of between 3.5 lux (e.g. dark limit of civil twilight) and 20 lux (e.g. public area with dark surroundings). Answer 1 if R3 is 1. \\ \hline
\multicolumn{1}{|c|}{R8} & \multicolumn{1}{c|}{1} & ...fully distinguishable when placed under an average illuminance of between 100 lux (e.g. very dark overcast day) and 1000 lux (e.g overcast day). \\ \hline
\multicolumn{1}{|c|}{R9} & \multicolumn{1}{c|}{1} & ...somewhat distinguishable when placed under an average illuminance of between 100 lux (e.g. very dark overcast day) and 1000 lux (e.g overcast day). Answer 1 if R5 is 1. \\ \hline
\multicolumn{1}{|c|}{R10} & \multicolumn{1}{c|}{1} & ...fully distinguishable when placed under an average illuminance of between 10000 lux and 25000 lux (e.g full daylight, not direct sun). \\ \hline
\multicolumn{1}{|c|}{R11} & \multicolumn{1}{c|}{1} & ...somewhat distinguishable when placed under an average illuminance of between 10000 lux and 25000 lux (e.g full daylight, not direct sun). Answer 1 if R7 is 1. \\ \hline
\multicolumn{1}{|c|}{R12} & \multicolumn{1}{c|}{1} & ...fully distinguishable when placed under an average illuminance of between 50000 and 130000 lux (e.g full daylight, sun overhead). \\ \hline
\multicolumn{1}{|c|}{R13} & \multicolumn{1}{c|}{1} & ...somewhat distinguishable when placed under an average illuminance of between 50000 and 130000 lux (e.g full daylight, sun overhead). Answer 1 if R9 is 1. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}READABILITY CONDITIONS - WEATHER\\ Accounting for dynamic adjustments if applicable, and under the best lighting conditions, all relevant eHMI(s) in this\\ proposal 33 feet away from the observer are fully readable...\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{R14} & \multicolumn{1}{c|}{1} & ...under a light rain (the average diameter of liquid water drops is no more than 0.10 inches ). \\ \hline
\multicolumn{1}{|c|}{R15} & \multicolumn{1}{c|}{1} & ...under moderate rain (the average diameter of liquid water drops is between 0.11 and 0.30 inches). \\ \hline
\multicolumn{1}{|c|}{R16} & \multicolumn{1}{c|}{1} & ...under a heavy rain (the average diameter of liquid water drops is more than 0.30 inches). \\ \hline
\multicolumn{1}{|c|}{R17} & \multicolumn{1}{c|}{1} & ...when lightning is present. \\ \hline
\multicolumn{1}{|c|}{R18} & \multicolumn{1}{c|}{1} & ...in dense fog (horizontal visibility reduced to under 1320 ft). \\ \hline
\multicolumn{1}{|c|}{R19} & \multicolumn{1}{c|}{1} & ...in medium fog (horizontal visibility is reduced to between 1321 ft and 5280 ft). \\ \hline
\multicolumn{1}{|c|}{R20} & \multicolumn{1}{c|}{1} & ...in light fog (horizontal visibility is not reduced to under 5280 ft ). \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}READABILITY CONDITIONS - DISTANCE\\ Under the best weather and light conditions for the relevant eHMI(s) in this proposal, they can be fully read and\\ understood by a person...\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{R21} & \multicolumn{1}{c|}{1} & 33 feet away. \\ \hline
\multicolumn{1}{|c|}{R22} & \multicolumn{1}{c|}{1} & 87 feet away. \\ \hline
\multicolumn{1}{|c|}{R23} & \multicolumn{1}{c|}{1} & 142 feet away. \\ \hline
\multicolumn{1}{|c|}{R24} & \multicolumn{1}{c|}{1} & 197 feet away. \\ \hline
\multicolumn{1}{|c|}{R25} & \multicolumn{1}{c|}{1} & 252 feet away. \\ \hline
\multicolumn{1}{|c|}{R26} & \multicolumn{1}{c|}{1} & 306 feet away. \\ \hline
\multicolumn{1}{|c|}{R27} & \multicolumn{1}{c|}{1} & 361 feet away. \\ \hline
\multicolumn{1}{|c|}{R28} & \multicolumn{1}{c|}{1} & 416 feet away. \\ \hline
\multicolumn{1}{|c|}{R29} & \multicolumn{1}{c|}{1} & 470 feet away. \\ \hline
\multicolumn{1}{|c|}{R30} & \multicolumn{1}{c|}{1} & 525 feet away. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}p{15.2cm}@{}}READABILITY CONDITIONS - ANGLE\\ If at any given time at least one of the eHMIs in this proposal is fully readable and understandable from all horizontal\\ angles, answer R33 through R42 with a 1. Otherwise, under the best possible conditions (weather, light, distance, etc),\\ can the average pedestrian or driver fully read and understand any and all given information displayed by any of the\\ relevant eHMIs in this proposal, when the horizontal angle formed by the direction of their sight and the element directly\\ displaying the information is...\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{R31} & \multicolumn{1}{c|}{1} & 90 degrees (direction of view perpendicular to the eHMI, observer in full-front view of it)? \\ \hline
\multicolumn{1}{|c|}{R32} & \multicolumn{1}{c|}{1} & Between 90 and 100 (90°, 100°{]}? \\ \hline
\multicolumn{1}{|c|}{R33} & \multicolumn{1}{c|}{1} & Between 100 and 110 (100°, 110°{]}? \\ \hline
\multicolumn{1}{|c|}{R34} & \multicolumn{1}{c|}{1} & Between 110 and 120 (110°, 120°{]}? \\ \hline
\multicolumn{1}{|c|}{R35} & \multicolumn{1}{c|}{1} & Between 120 and 130 (120°, 130°{]}? \\ \hline
\multicolumn{1}{|c|}{R36} & \multicolumn{1}{c|}{1} & Between 130 and 140 (130°, 140°{]}? \\ \hline
\multicolumn{1}{|c|}{R37} & \multicolumn{1}{c|}{1} & Between 140 and 150 (140°, 150°{]}? \\ \hline
\multicolumn{1}{|c|}{R38} & \multicolumn{1}{c|}{1} & Between 150 and 160 (150°, 160°{]}? \\ \hline
\multicolumn{1}{|c|}{R39} & \multicolumn{1}{c|}{1} & Between 160 and 170 (160°, 170°{]}? \\ \hline
\multicolumn{1}{|c|}{R40} & \multicolumn{1}{c|}{1} & More than 170 degrees from it? \\ \hline

\end{tabular}
%\end{table*}

==> questionnaires/qr2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
%\begin{table*}[ht]
\begin{tabular}{|p{0.5cm} | p{0.5cm} | p{15.2cm}|}
\hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{p{15cm}}READABILITY CONDITIONS - ANGLE\\ Under the best possible conditions (weather, light, distance, etc), the average pedestrian or driver can fully read and understand any and all given information displayed by any of the relevant eHMIs in this proposal, when the horizontal angle formed by the direction of their sight and the element directly displaying the information is...\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{R26} & \multicolumn{1}{c|}{1} & 90 degrees (direction of view perpendicular to the eHMI, pedestrian in full-front view of it). \\ \hline
\multicolumn{1}{|c|}{R27} & \multicolumn{1}{c|}{1} & Between 90 and 100 (90°, 100°{]}. \\ \hline
\multicolumn{1}{|c|}{R28} & \multicolumn{1}{c|}{1} & Between 100 and 110 (100°, 110°{]}. \\ \hline
\multicolumn{1}{|c|}{R29} & \multicolumn{1}{c|}{1} & Between 110 and 120 (110°, 120°{]}. \\ \hline
\multicolumn{1}{|c|}{R30} & \multicolumn{1}{c|}{1} & Between 120 and 130 (120°, 130°{]}. \\ \hline
\multicolumn{1}{|c|}{R31} & \multicolumn{1}{c|}{1} & Between 130 and 140 (130°, 140°{]}. \\ \hline
\multicolumn{1}{|c|}{R32} & \multicolumn{1}{c|}{1} & Between 140 and 150 (140°, 150°{]}. \\ \hline
\multicolumn{1}{|c|}{R33} & \multicolumn{1}{c|}{1} & Between 150 and 160 (150°, 160°{]}. \\ \hline
\multicolumn{1}{|c|}{R34} & \multicolumn{1}{c|}{1} & Between 160 and 170 (160°, 170°{]}. \\ \hline
\multicolumn{1}{|c|}{R35} & \multicolumn{1}{c|}{1} & More than 170 degrees from it. \\ \hline
\end{tabular}
%\end{table*}

==> questionnaires/qs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
%\begin{table*}[ht]
\caption{Standardization Questionnaire}
\label{tab:QS_table}
\begin{adjustwidth}{-2cm}{-2cm}
\centering
\tiny
\begin{tabular}{|p{0.5cm} | p{0.5cm} | p{15.2cm}|}
\hline
\rowcolor[HTML]{CCCCCC} 
\multicolumn{3}{|c|}{\cellcolor[HTML]{CCCCCC}\textbf{STANDARDIZATION}} \\ \hline
\rowcolor[HTML]{CCCCCC} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{CCCCCC}\textbf{ID}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{PTS}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{QUESTION}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{GENERAL} \\ \hline
\multicolumn{1}{|c|}{S1} & \multicolumn{1}{c|}{1} & PLACEMENT: The proposal does not specify the eHMI's specific placement on the vehicle (e.g. grill, windshield, door, etc) \\ \hline
\multicolumn{1}{|c|}{S2} & \multicolumn{1}{c|}{1} & ON STATE: The proposed eHMI has a display that can turn on and off. \\ \hline
\multicolumn{1}{|c|}{S3} & \multicolumn{1}{c|}{4} & USES TEXT: The proposed eHMI makes use of text, requiring standardization of font, letter spacing, color, and size. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}FRAME\\ If this eHMI does not use a frame, answer S4 through S6 with “0”.\\ If this eHMI doesn't specify whether it uses a frame, answer S4 through S6 with "1"\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{S4} & \multicolumn{1}{c|}{1} & FRAME COLOR: The eHMI has a frame around it that can be made in more than one color. \\ \hline
\multicolumn{1}{|c|}{S5} & \multicolumn{1}{c|}{1} & FRAME THICKNESS: The eHMI has a frame around it that can be made in more than one thickness. \\ \hline
\multicolumn{1}{|c|}{S6} & \multicolumn{1}{c|}{1} & FRAME BRIGHTNESS: The eHMI has a frame around it that lights up at more than one possible brightness. \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}BACKGROUND\\ If this eHMI does not use a background, answer S7 through S9 with “0”.\\ If this eHMI doesn't specify whether it uses a frame, answer S7 through S9 with "1".\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{S7} & \multicolumn{1}{c|}{1} & BACKGROUND COLOR: The eHMI has a uniform background that can be made in more than one possible color, but does not change colors dynamically. \\ \hline
\multicolumn{1}{|c|}{S8} & \multicolumn{1}{c|}{1} & BACKGROUND CONTENT: The eHMI uses a pattern or image as a background, but cannot change it dynamically \\ \hline
\multicolumn{1}{|c|}{S9} & \multicolumn{1}{c|}{Bcc} & BACKGROUND CHANGE CONDITIONS (Bcc: the number of conditions that could trigger a change in the background.) \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}PICTOGRAM\\ If this eHMI does not use pictograms, answer S10 through S15 with “0”.\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{S10} & \multicolumn{1}{c|}{Pdc} & PICTOGRAM DESIGN CHANGE CONDITIONS (Pdc: the number of conditions that could trigger a change in the pictogram design.) \\ \hline
\multicolumn{1}{|c|}{S11} & \multicolumn{1}{c|}{1} & PICTOGRAM COLOR: The pictogram can be made in multiple colors, and as such requires color standardization. \\ \hline
\multicolumn{1}{|c|}{S12} & \multicolumn{1}{c|}{Pcc} & PICTOGRAM COLOR CHANGE CONDITIONS (Pcc: the number of conditions that could trigger a change in the pictogram color.) \\ \hline
\multicolumn{1}{|c|}{S13} & \multicolumn{1}{c|}{Psc} & PICTOGRAM SIZE CHANGE CONDITIONS (Psc: the number of conditions that could trigger a change in the pictogram size.) \\ \hline
\multicolumn{1}{|c|}{S14} & \multicolumn{1}{c|}{Pmc} & PICTOGRAM MARGIN CHANGE CONDITIONS (Pmc: the number of conditions that could trigger a change in the pictogram margins.) \\ \hline
\multicolumn{1}{|c|}{S15} & \multicolumn{1}{c|}{Pv - 1} & PICTOGRAM VARIANTS (Pv: all the possible states of this display, made from the possible combinations of pictogram design, color, size, and margins.) \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}TEXT\\ If this eHMI does not use text, answer S16 through S22 with “0”.\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{S16} & \multicolumn{1}{c|}{Ttc} & TEXT CHANGE CONDITIONS (Ttc: the number of conditions that could trigger a change in the text content.) \\ \hline
\multicolumn{1}{|c|}{S17} & \multicolumn{1}{c|}{1} & TEXT COLOR: The text can be made to display multiple colors, and as such requires color standardization. \\ \hline
\multicolumn{1}{|c|}{S18} & \multicolumn{1}{c|}{Tcc} & TEXT COLOR CHANGE CONDITIONS (Tcc: the number of conditions that could trigger a change in the text color.) \\ \hline
\multicolumn{1}{|c|}{S19} & \multicolumn{1}{c|}{Tf} & TEXT FONT CHANGE CONDITIONS (Tf: the number of conditions that could trigger a change in the text typeface.) \\ \hline
\multicolumn{1}{|c|}{S20} & \multicolumn{1}{c|}{Ts} & TEXT SIZE CHANGE CONDITIONS (Ts: the number of conditions that could trigger a change in the text size.) \\ \hline
\multicolumn{1}{|c|}{S21} & \multicolumn{1}{c|}{Tm} & TEXT MARGIN CHANGE CONDITIONS (Tm: the number of conditions that could trigger a change in the text margins.) \\ \hline
\multicolumn{1}{|c|}{S22} & \multicolumn{1}{c|}{Tv - 1} & TEXT VARIANT CHANGE CONDITIONS (Tv: all the possible states of this display, made from the possible combinations of: Text content, text color, text font, font size, font spacing, and text margins. ) \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}ANIMATION\\ If this eHMI does not use animations or motions, answer S26 with “0”\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{S23} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}$\frac{Ams}{1000}$\\ $+ Aks$\\$+ Arc$\end{tabular}} & \begin{tabular}[c]{@{}p{15.2cm}@{}}TOTAL MOTION PLAYTIME: (Ams: The sum of all milliseconds taken by each individual animation that this eHMI plays \\(e.g. swiping, growing, fade in, etc), rounding up.\\ Aks: The number of kinematic actions that this eHMI employs.\\ Arc: The amount of animations that repeat intermittently.).\end{tabular} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{\begin{tabular}[c]{@{}l@{}}SOUND\\ If this eHMI does not use sound, answer S27 through S29 with “0”\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{S24} & \multicolumn{1}{c|}{Sc} & SOUND COUNT (Sc: the amount of sounds used by this eHMI. ) \\ \hline
\multicolumn{1}{|c|}{S25} & \multicolumn{1}{c|}{Ssc} & SPEAKERS COUNT (Ssc: The amount of speakers used by this eHMI.) \\ \hline
\multicolumn{1}{|c|}{S26} & \multicolumn{1}{c|}{Sc} & PITCH AND VOLUME (Sa: the amount of sounds used by this eHMI.) \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}} & \textbf{OTHERS} \\ \hline
\multicolumn{1}{|c|}{S27} & \multicolumn{1}{c|}{Ot} & OTHER TRIGGERS (Ot: the amount of conditions that trigger any change in the eHMI otherwise not mentioned in this questionnaire.) \\ \hline
\end{tabular}
\end{adjustwidth}
%end{table}

==> results/accessibility_results.tex <==
\subsection{Accessibility Scores}
None of the proposals evaluated make use of sound components (\(A_{4} = 0, A_{{35 to 41}} = 0\)) or tactile components (\(A_{3} = 0, A_{{35}} = 0\)), nor do they employ imagery that could be distressing (\(A_{{64 to 68}} = 1\)) or psychologically offensive (\(A_{{69 to 73}} = 1\)). Based on the results of \cite{de_clercq_external_2019}, all of the presented proposals provide enough time to the observer to be understood (\(A_{{48}} = 1\)). The results of this evaluation can be seen in Table \ref{tab:result3_table1}.

\subsubsection{Vehicle Kinematics as Indication (No eHMI)} 
The vehicle kinematics do not use pictograms (\(A_{1_{No eHMI}} = 0, A_{{9 to 17}_{No eHMI}} = 0\)), or text (\(A_{2_{No eHMI}} = 0, A_{{18 to 29}_{No eHMI}} = 0, A_{{47}_{No eHMI}} = 0, A_{{52 to 53}_{No eHMI}} = 1\)). While a vehicle may make a screeching sound as it stops, this is not mentioned in the literature as a relevant factor in how pedestrians interact with a yielding vehicle.

Using the sides of the vehicle as the 'display' means that while the placement of information is consistent (\(A_{7_{No eHMI}} = 1\)), it is also affected by the size of said vehicle (\(A_{5_{No eHMI}} = 0\)). No measures are taken to prevent the creation of shadows on this part of the vehicle (\(A_{8_{No eHMI}} = 0\)), and since the kinematics are observed through the chassis of the vehicle, some types of vehicles such a emergency ones may have additional visual clutter that difficult the reading of the motion (\(A_{6_{No eHMI}} = 0\)). The vehicle kinematics do not rely on color to communicate information (\(A_{30_{No eHMI}} = 1, A_{32_{No eHMI}} = 1, A_{33_{No eHMI}} = 1\)), but the color of the vehicle may be one commonly confused by color blind people (\(A_{31_{No eHMI}} = 0\)) such as red (\(A_{44_{No eHMI}} = 0\)). This proposal does not use flashing lights (\(A_{42_{No eHMI}} = 1, A_{43_{No eHMI}} = 1\)) or animations (\(A_{45_{No eHMI}} = 1, A_{46_{No eHMI}} = 1\)). Since the color of the eHMI is the same as its paint job, questions regarding that aspect are non-applicable (\(A_{34_{No eHMI}} = 0\)).

According to the results observed by Moore et al \cite{moore_case_2019}, pedestrians mainly rely on vehicle kinematics to determine when the vehicle is yielding to them. However, the motion is only and solely communicated implicitly (\(A_{{49 to 51}_{No eHMI}} = 0 \)). This method of communication is universal (\(A_{{54 to 58}_{No eHMI}} = 1\)), but it may hold a different meaning or be read differently depending on the situational context (\(A_{{59 to 63}_{No eHMI}} = 0\)).

\subsubsection{Front Braking Lights (FBL)} 
These do not use pictograms (\(A_{1_{FBL}} = 0, A_{{9 to 17}_{FBL}} = 0\)), or text (\(A_{2_{FBL}} = 0, A_{{18 to 29}_{FBL}} = 0, A_{{47}_{FBL}} = 0, A_{{52 to 53}_{FBL}} = 1\)). Since all vehicles have headlights, frontal brake lights can be consistently placed regardless of vehicle type or size (\(A_{5_{FBL}} = 1\)), the information is always displayed in the same eHMI (\(A_{7_{FBL}} = 1\)). The placement of frontal brake lights is close to the vehicle headlights, which creates visual clutter that may confuse an observer (\(A_{6_{FBL}} = 0\)). Headlights take measures to prevent the creation of shadows that may obscure them (\(A_{8_{FBL}} = 1\)).

Not the color, but the brightness state of the lights determine the intent of the vehicle (\(A_{30_{FBL}} = 1\)), and the sole color cyan in the proposal (\(A_{32_{FBL}} = 1, A_{44_{FBL}} = 1\)) does not fall within the most common color blind colors (\(A_{31_{FBL}} = 1\)). It may also be adjusted to fit local regulations (\(A_{33_{FBL}} = 1\)), although it does not have a way to ensure it doesn't blend with the rest of the vehicle (\(A_{34_{FBL}} = 1\)). The lights do not flash (\(A_{42_{FBL}} = 1, A_{43_{FBL}} = 1\)) nor do they employ any animations (\(A_{45_{FBL}} = 1, A_{46_{FBL}} = 1\)). 

The information communicated relates to the speed of the vehicle instead of its yielding decision, meaning it is presented implicitly (\(A_{50_{FBL}} = 0\)) and in only one way (\(A_{49_{FBL}} = 0\)) that is exocentric to the observer (\(A_{51_{FBL}} = 0\)). Considering the proliferation of tail lights in modern vehicles, the meaning of frontal brake lights, while new, can be considered universal (\(A_{{54 to 58}_{FBL}} = 1\)), although not independent from context since it may signal yielding or a simple slowing down of the vehicle (\(A_{{59 to 63}_{FBL}} = 1\)).

\subsubsection{Knight Rider Display (KRD)}
This display uses an animated, one dimensional pictogram (\(A_{1_{KRD}} = 1\)), but no text (\(A_{2_{KRD}} = 0, A_{{18 to 29}_{KRD}} = 0, A_{{47}_{KRD}} = 0, A_{{52 to 53}_{KRD}} = 1\)). Part of the placement is on the bumper which is not a cluttered space (\(A_{6_{KRD}} = 1\)), but it is one that can be affected or changed by vehicle type (\(A_{5_{KRD}} = 0\)). This proposal consistently places the display on the bumper (\(A_{7_{KRD}} = 1\)). The sample for this proposal is based on the sign display in \cite{ledsigncity_car_nodate}, which adjusts its brightness based on the environment to prevent shadows (\(A_{8_{KRD}} = 1\)) and glare (\(A_{14_{KRD}} = 1\)).

The pictogram is made up of identical upright straight thick bold cyan lights (\(A_{{10 to 12}_{KRD}} = 1\)) over a black background (\(A_{{15 to 17}_{KRD}} = 1\)), inside of a silver frame. This combination of light and dark should provide enough contrast from the vehicle paint job (\(A_{34_{KRD}} = 1\)) and surrounding elements (\(A_{9_{KRD}} = 0\)). The sweeping motion is also distinguishable from the static motion (\(A_{13_{KRD}} = 1\)). It does not rely on color to communicate information (\(A_{30_{KRD}} = 1\)) or use a color that is commonly problematic to color blind people (\(A_{31_{KRD}} = 1\)) such as red (\(A_{32_{KRD}} = 1, A_{44_{KRD}} = 1\)). The color can be changed during manufacturing (\(A_{33_{KRD}} = 1\)).

Each segment of the Knight Rider Display may flash (\(A_{42_{KRD}} = 0\)) but no more than three times per second (\(A_{43_{KRD}} = 1\)). While this proposal uses animations, these are all simple (\(A_{45_{KRD}} = 1\)) and not featuring any elements scrolling at different speeds (\(A_{46_{KRD}} = 1\)). 

While this proposal features two eHMIs, they both present information in the same exocentric way (\(A_{49_{KRD}} = 0, A_{51_{KRD}} = 0\)). The eHMIs only play their respective animation when the vehicle intends to yield, making the communication explicit (\(A_{{50}_{KRD}} = 0\)). This method of communication is potentially not universal, and based on an American television show from 1982 \cite{larson_knight_1982} (\(A_{{54 to 58}_{KRD}} = 0\)). There isn't enough data to determine if the animation of this proposal may hold a different meaning based on the surroundings of the vehicle (\(A_{{59 to 63}_{KRD}} = 0\)).

\subsubsection{Bumper Smile Display (BSD)}
This proposal has a single eHMI: A LED display that uses the pictogram of a smile (\(A_{{1}_{BSD}} = 1\)) to communicate yielding intent. No text is employed (\(A_{2_{BSD}} = 0, A_{{18 to 29}_{BSD}} = 0,  A_{{47}_{BSD}} = 0, A_{{50}_{BSD}} = 1, A_{{51 to 53}_{BSD}} = 1\)). The eHMI is consistently placed on the bumper (\(A_{7_{BSD}} = 1\)), which is not a cluttered space (\(A_{6_{BSD}} = 1\)) but one that can change based on vehicle type (\(A_{5_{BSD}} = 0\)). The sample for this proposal is based on the sign display in \cite{ledsigncity_car_nodate}, which adjusts its brightness based on the environment to prevent shadows (\(A_{8_{BSD}} = 1\)) and glare (\(A_{14_{BSD}} = 1\)).

The pictogram of the smile uses a curved (\(A_{12_{BSD}} = 0\)) upright (\(A_{10_{BSD}} = 1\)), thick, uniform, and bold cyan line (\(A_{11_{BSD}} = 1\)) over a black background (\(A_{{15 to 17}_{BSD}} = 1\)), inside of a silver frame that distinguishes it from the rest of the vehicle (\(A_{{34}_{BSD}} = 1\)). This combination of light and dark should provide enough contrast with the vehicle paintjob and other surrounding elements (\(A_{9_{BSD}} = 0\)). The straight and the curved pictogram are distinguishable from each other (\(A_{13_{BSD}} = 1\)). It does not rely on color to communicate information (\(A_{30_{BSD}} = 1\)) or use a color that is commonly problematic to color blind people (\(A_{31_{BSD}} = 1\)) such as red (\(A_{44_{BSD}} = 1\)). The color used in this proposal is cyan (\(A_{{32}_{BSD}} = 1\)) and can be adjusted during manufacturing (\(A_{{33}_{BSD}} = 1\)).

While this proposal features a display, it does not flash (\(A_{{42 to 43}_{BSD}} = 1\)), as it just switches between two states instead of employing any animations (\(A_{{45 to 46}_{BSD}} = 1\)). Information is always presented in one exocentric way (\(A_{{49}_{BSD}} = 0, A_{{51}_{BSD}} = 0\)) but not in a way that is explicitly stated to the observer (\(A_{{50}_{BSD}} = 0\)).

Smiles are not a universal symbol of friendliness (\(A_{{54 to 58}_{BSD}} = 0\)) that may take on a different meaning depending on context \cite{krys_be_2015} (\(A_{{59 to 63}_{BSD}} = 0\)).

\subsubsection{Bumper Text Display (BTD)}
This proposal employs text (\(A_{2_{BTD}} = 1\)) instead of pictograms  (\(A_{1_{BTD}} = 0, A_{{9 to 14}_{BTD}} = 0\)). While some variants of the proposal place the text on the windshield, this specific example places it on the bumper (\(A_{7_{BTD}} = 1\)), which is a cluttered space (\(A_{6_{BTD}} = 0\)) that can change based on vehicle type (\(A_{5_{BTD}} = 0\)). This display adjusts its brightness based on the environment to prevent shadows (\(A_{8_{BTD}} = 1\)) and glare (\(A_{25_{BTD}} = 1\)) \cite{ledsigncity_car_nodate}.

The eHMI displays letters over a black background (\(A_{{15 to 18}_{BTD}} = 1\)), which contrasts with the adjustable cyan letters (\(A_{{20}_{BTD}} = 1, A_{{31 to 33}_{BTD}} = 1\)) and the rest of the vehicle (\(A_{{34}_{BTD}} = 1\)). The text is displayed upright (\(A_{{19}_{BTD}} = 1\)), using the bold Helvetica font which uses straight, uniform thick lines (\(A_{{20 to 22}_{BTD}} = 1\)) with wide horizontal proportions (\(A_{{27}_{BTD}} = 1\)) to display distinct characters (\(A_{{23}_{BTD}} = 1\)) with prominent ascenders, descenders, and open counterforms (\(A_{{24}_{BTD}} = 1\)).

The text displayed is ``Walk' and ``Don't walk', making use of initial uppercase letters (\(A_{{26}_{BTD}} = 1\)) and simple language (\(A_{{52}_{BTD}} = 1, A_{53_{BTD}} = 1\)). It does not rotate (\(A_{{28}_{BTD}} = 1\)), include hyphens or em dashes (\(A_{{29}_{BTD}} = 1\)), or rely on color to communicate information (\(A_{{30}_{BTD}} = 1\)). The display only uses the color black and cyan (\(A_{{31}_{BTD}} = 1, A_{44_{BTD}} = 1\)), and it does not feature flashing lights (\(A_{{42 to 43}_{BTD}} = 1\)) or animations (\(A_{{45 to 46}_{BTD}} = 1\)). 

The ``Walk' message is explicitly egocentric to the pedestrian (\(A_{{50 to 51}_{BTD}} = 1\)) when the vehicle starts its yielding behavior. Based on the results in \cite{de_clercq_external_2019}, a pedestrian should be able to read and interpret the instructions in the time given by the vehicle (\(A_{{47}_{BTD}} = 1\)). The language used is plain and idiom-free (\(A_{{55 to 53}_{BTD}} = 1\)). 

The instructions are not presented in another way (\(A_{{49}_{BTD}} = 0\)). Text relies on language to be understood, meaning that it is not applicable to the cultural or contextual sections of the questionnaire (\(A_{{54 to 58}_{BTD}} = 0, A_{{59 to 63}_{BTD}} = 1\)).



%The animation is described to be (TODO) seconds in length, while the average vehicle takes (TODO) seconds to go from (TODO) to a full stop \cite{}, giving the pedestrian (TODO) time see the full animation, interpret it, and act accordingly (\(A_{47_{KRD}} = TODO\)). 

\input{tables/results3_1}

\input{tables/results3_2}

==> results/constant_communication_results.tex <==


\subsection{Constant Communication Scores}
%This scores this proposal a mere 2 points on Table \ref{tab:result5_table}.

\subsubsection{Vehicle Kinematics as Indication (No eHMI)} 
By themselves, the vehicle kinematics can communicate motion (\(CC_{1_{No eHMI}} = 1\)) and acceleration (\(CC_{3_{No eHMI}} = 1, CC4_{4_{No eHMI}} = 1\)). Vehicle kinematics do not explicitly communicate to observers the many intricacies and possible errors of the navigation system. It is also limited to situations where a vehicle may or may not yield for a pedestrian. 

\subsubsection{Front Braking Lights (FBL)} 
The Frontal Braking Lights can communicate when the vehicle is slowing down (\(CC_{3_{FBL}} = 1\)), however it doesn't have a state exclusive to when the vehicle is in motion or for when the vehicle is accelerating.

\subsubsection{Knight Rider Display (KRD)}
Since this display does not turn on when a person is driving the vehicle, it communicates when the vehicle is in autonomous mode (\(CC_{5_{KRD}} = 1\)), but it does not explicitly communicate otherwise. This display also remains solid when the vehicle is yielding to a pedestrian (\(CC_{15_{KRD}} = 1\)) and plays a swiping animation when it's not yielding to them (\(CC_{15_{KRD}} = 1\)). While the display communicates when the vehicle is slowing down as part of its yielding behavior, it does not explicitly communicate when it's slowing down for another reason.  

\subsubsection{Bumper Smile Display (BSD)}
Similarly to the Knight Rider Display, the Bumper Smile Display can communicate when the vehicle is in autonomous mode (\(CC_{5_{BSD}} = 1\)), when it is yielding to a pedestrian (\(CC_{14_{BSD}} = 1\)), and when it is not (\(CC_{15_{BSD}} = 1\)), but it does not communicate additional information.

\subsubsection{Bumper Text Display (BTD)}
The technology in the proposal can be used to display a wide variety of information, but within the scope of this evaluation and the description given, it only communicates the vehicle is in autonomous mode (\(CC_{5_{BTD}} = 1\)), when it is yielding to a pedestrian (\(CC_{14_{BTD}} = 1\)), and when it is not yielding to a pedestrian (\(CC_{15_{BTD}} = 1\)). 



%\begin{table}[ht]
%\end{table}



\input{tables/results5}





%
%
%

==> results/cost_effectiveness_results.tex <==
\subsection{Cost Effectiveness Scores}
None of the proposals outline a manufacturing, installation, maintenance, or operation cost. To nonetheless present a frame of reference, this section uses information available on similar technology to produce an estimate. All adjustment for inflation were made using the CPI Inflation Calculator by the United Stated Bureau of Labor Statistics \cite{us_bureau_of_labor_statistics_cpi_nodate}, using December 2022 as the target date. 
As stated in Appendix, whenever a range is given, the value used is the median of that range, and whenever the answer is unknown, the highest value in the questionnaire for that eHMI is used instead. 

\subsubsection{No eHMI} 
Since the kinematics of a vehicle are part of the normal behavior of modern vehicles, there is no additional cost to implement it, maintain it, or develop it.

\begin{table}[ht]
\input{tables/results2_1}
\end{table}

\subsubsection{Tail Lights} 
Frontal Brake Lights use the same technology as tail braking lights. The cheapest replacement for a single tail brake light with light bulb in 2024 is \$20.99 in carparts.com \cite{noauthor_replacement_nodate}. After accounting for both lights, and adjusting for inflation, it makes \({CE_{1_{Brake Light}}} = 39.68\). 
Repair Pal estimates the labor cost of replacing a tail light to be between \$40 and \$51 \cite{noauthor_brake_nodate}, which makes \(CE_{3_{Brake Light}} = 43.00\) after calculating the median and adjusting for inflation. The manufacturing cost is disclosed, forcing us to use the same cost as an existing vehicle \(CE_{2_{Brake Light}} = CE_{3_{Brake Light}} = 43.00\).
A car light bulb has a lifetime of between 14 and 42 months, according to Michael \cite{michael_how_2019}. By using the following equation

\begin{equation} \label{yearly_cost_equation}
    CE_4 = \frac{CE_1 + \frac{(CE_2 + CE_3)}{2}}{{Median Lifetime in Years}}
\end{equation}
where \({Median Lifetime in Years} \approx 2.33\), we can conclude that \(CE_{4_{Brake Light}} \approx 53.94\).
Information on the operating costs of tail lights was not available, so the highest value in this category was chosen, making \(CE_{5_{Brake Light}} = 53.94\).
%an estimate was calculated by determining the energy consumption of the lights multiplying the amounts of vehicle operation by the wattage of the eHMI. and the cost of operating them wasforcing us to use the highest value so far, making \(CE_{5_{Brake Light}} = 699.06\).

\begin{table}[ht]
\input{tables/results2_2}
\end{table}

\subsubsection{LED Displays}
The Knight Rider Display, Bumper Smile Display, and Bumper Text Display all make use of LED screens to show pictograms or text to the observer. These can be compared to LED advertisement signs placed on vehicles, as they both must endure the elements and be visible to observers. 

According to LED Sign City \cite{ledsigncity_car_nodate}, the cost of a single Taxi Top LED sign ranges from \$3900.00 and \$4875.00. After calculating the median and adjusting for inflation, this makes \(CE_{1_{LED Display}} = 4606.90\).

LED Sign City includes installation cost with the purchase, making \(CE_{2_{LED Display}} = 0.00\) and \(CE_{3_{LED Display}} = 0.00\).

These signs have a warranty of 2 years. Using Equation (\ref{yearly_cost_equation}),  \(CE_{4_{LED Display}} = 2303.45\).
The LED signs in \cite{ledsigncity_car_nodate} require up to 570 watts. According to Gross, the average person living in the United States spends at least 17600 minutes \(\approx293.33 hours\) driving each year \cite{gross_americans_2016}. Since all examples making use of this display have it on at all times during driving, we calculated the energy consumption of the display by using the equation 
\begin{equation} \label{W to kWh}
    {kWh} = \frac{W \times {hours}}{1000}
\end{equation}
where \(W = 570\) and \({hours} \approx 293.33\). The operation cost was then calculated using
    \begin{equation} \label{kWh to usd}
        {CE5_{x}} = {kWh} \times {rate_{2022}}
    \end{equation}
where \({rate_{2022}} = 0.165 \frac{USD}{kWh}\), which is the average price of a kWh in the United States in December of 2022 according to the United States Bureau of Labor Statistics \cite{us_bureau_of_labor_statistics_average_2022}, making \(CE_{5_{LED Display}} \approx 27.59\)

\begin{table}[ht]
\input{tables/results2_3}
\end{table}

\subsubsection{LED Light Array}
The Knight Rider display makes use of seven additional LED lights that work in conjunction with its main display. These can be compared to 5mm color LED lamps, like the ones in LED Supply \cite{noauthor_5mm_nodate}.
Each lamp costs \$1.20 each, which can be adjusted for inflation to \(cost_{LED Light Array} = 1.13\). Using the following equation
    \begin{equation} \label{cost_of_led_lights}
        {CE_{1_{LED Light Array}}} = 7 \times {cost_{LED Light}}
    \end{equation}
results in \(CE_{1_{LED Light Array}} = 7.91\).

The yearly operating cost of a single LED light bulb needs to be calculated first by using the equation
    \begin{equation} \label{power_equation}
        W = {Voltage} \times {Current}
    \end{equation}
where \(Voltage = 3.5V\) and \(Current = 0.03A\), resulting in \(W = 0.105W\). The energy used by the light was calculated by applying Equation (\ref{W to kWh}). Unlike the LED display, the lights are not on when the vehicle is in motion, but since no data can be found on how much time a vehicle would spend telling a pedestrian to cross we used the same value for time as with the display, which is to say \({hours} \approx 293.33\), this results in \(kWh \approx 0.03kWh\). Using the same value for \(rate\) as before and Equation (\ref{kWh to usd}), we determined that the average yearly operating cost of a single LED lamp is \$0.00495, which means \(CE_{5_{LED Light Array}} = 0.03465 \approx 0.03\) for all seven lights in conjunction.

Since this proposal hasn't been implemented, there was not an appropriate comparison for installation costs of the light. We instructed, we made it so \(CE_{2_{LED Light Array}} = 1.13\) and \(CE_{3_{LED Light Array}} = 1.13\).

According to Inline Lighting Electrical, a LED bulb will last, on average, 25000 hours before it produces 70\% of its original light \cite{noauthor_life_nodate}. Considering that the average person living in the United States drives \(\approx293.33\) hours per year, it would take \(\approx85.23 years\) before the average LED light bulb on this eHMI needs to be replaced. Using Equation (\ref{yearly_cost_equation}), this means \(CE_{4_{LED Light Array}} \approx 0.01\).

\begin{table}[ht]
\input{tables/results2_4}
\end{table}

\subsubsection{Vehicle Kinematics as Indication (No eHMI)}
The kinematic motion doesn't use any additional cost, so \(CE_{{1 to 5}_{No eHMI}} = 0\).

\subsubsection{Frontal Brake Lights (FBL)}
The Frontal Braking Light proposal uses solely the breaking light technology so its score is calculated using the equation 
    \begin{equation} \label{frontal_brake_light_cost_equation}
        CE_{n_{FBL}} = CE_{n_{Brake Light}}
    \end{equation}
    
\subsubsection{Knight Rider Display (KRD)}
The Knight Rider Display  uses the following equation to calculate its answers:
    \begin{equation} \label{knight_rider_cost_equation}
        CE_{n_{KRD}} = CE_{n_{LED Display}} + CE_{n_{LED Light Array}}
    \end{equation}

\subsubsection{Bumper Smile Display (BSD) and Bumper Text Display (BTD)}
Both the Bumper Smile Display and Bumper Text Display use the same technology so they use the equation
    \begin{equation} \label{BSD_and_BTD_cost_equation}
        CE_{n_{BSD}} = CE_{n_{BTD}} = CE_{n_{LED Display}}
    \end{equation}

\subsubsection{Results}
The results for this section can be seen in Table \ref{tab:result2_table}
\begin{table}[ht]
\input{tables/results2}
\end{table}

==> results/ease_of_understanding_results.tex <==
\subsection{Ease of Understanding Scores}
This evaluation uses the \textit{feel-safe percentages} \((FSP)\) given in \cite[Fig.~9]{de_clercq_external_2019}, rounded to the nearest whole number. Since the participants in that experiment had a mean age of 24.57 years, these values are used for the question corresponding to adult pedestrians.

Since the study does not produce other demographic information, no other questions were answered in this scenario.

%\begin{table}[ht]
\input{tables/results4}
%\end{table}

==> results/positioning_results.tex <==
\subsection{Positioning Scores}
For this analysis, the purpose of all of these eHMI is solely to communicate to pedestrians and drivers looking at the vehicle's front of the it's intent to yield to a pedestrian (\(P_{34} = 0, P_{38} = 0, P_{39} = 0\)). All of these proposals are symmetrical (\(P_{1} = 1\)), and none are placed on the roof of the vehicle (\(P_{2} = 1\)). Results can be seen on Table \ref{tab:result6_table}.

\subsubsection{Vehicle Kinematics as Indication (No eHMI)} 
Both sides of the vehicle serve as the display of this proposal, this includes both pairs of fenders (\(P_{5_{No eHMI}} = 2, P_{15_{No eHMI}} = 2\)), pairs of doors (\(P_{14_{No eHMI}} = 2, P_{23_{No eHMI}} = 2\)), pairs of wheels (\(P_{18_{No eHMI}} = 2, P_{24_{No eHMI}} = 2\)), windshield rails (\(P_{17_{No eHMI}} = 2\)), back window rails (\(P_{8_{No eHMI}} = 2\)), headlights (\(P_{21_{No eHMI}} = 2\)), rocker panels (\(P_{26_{No eHMI}} = 2\)), side mirrors (\(P_{28_{No eHMI}} = 2, P_{29_{No eHMI}} = 2\)), and tail lights (\(P_{31_{No eHMI}} = 2\)). 

This makes \(P_{33_{No eHMI}} = 1\), \(P_{35_{No eHMI}} = 1\), \(P_{36_{No eHMI}} = 1\), \(P_{37_{No eHMI}} = 1\), and \(P_{40_{No eHMI}} = 1\).

\subsubsection{Front Braking Lights (FBL)} 
These are placed under the headlights, on the front bumper (\(P_{12_{FBL}} = 2\)). This makes \(P_{33_{FBL}} = 1\), \(P_{35_{FBL}} = 1\), \(P_{36_{FBL}} = 0\), \(P_{37_{FBL}} = 0\), and \(P_{40_{FBL}} = 1\).

\subsubsection{Knight Rider Display (KRD)}
While this proposal has two separate elements, both of these serve the same purpose, so they are treated as the same for this section of the evaluation. One of the displays is on the front bumper (\(P_{12_{KRD}} = 2\)) and front plate (\(P_{16_{KRD}} = 2\)), while the other is on the hood of the vehicle (\(P_{22_{KRD}} = 2\)). This makes \(P_{33_{KRD}} = 1\), \(P_{35_{KRD}} = 1\), \(P_{36_{KRD}} = 0\), \(P_{37_{KRD}} = 0\), and \(P_{40_{KRD}} = 1\).

\subsubsection{Bumper Smile Display (BSD)}
This display is on the front bumper (\(P_{12_{BSD}} = 2\)) and front plate (\(P_{16_{BSD}} = 2\)). This makes \(P_{33_{BSD}} = 1\), \(P_{35_{BSD}} = 1\), \(P_{36_{BSD}} = 0\), \(P_{37_{BSD}} = 0\), and \(P_{40_{BSD}} = 1\).


\subsubsection{Bumper Text Display (BTD)}
This display is on the front bumper (\(P_{12_{BTD}} = 2\)) and front plate (\(P_{16_{BTD}} = 2\)). This makes \(P_{33_{BTD}} = 1\), \(P_{35_{BTD}} = 1\), \(P_{36_{BTD}} = 0\), \(P_{37_{BTD}} = 0\), and \(P_{40_{BTD}} = 1\).


\mycomment
{

The results of this portion were based on the samples in Fig. \ref{fig:baseline_example} through Fig. \ref{fig:text_example}, and using the observations by Troel-Madec et al \cite{troel-madec_ehmi_2019}, where the observer is positioned facing the front-left and front-right side of the vehicle. If the 'visible percentage' was found to be above 40\% for a scenario, it was considered visible under those circumstances. The results can be seen on Table \ref{tab:result6_table}. 

%%More specific research must be done in this area, as simulations are imperfect and do not include other elements in the street that could interfere with the reading of the motion (lamp posts, newspaper stands, fire hydrants, etc). It must be noted that in \cite{troel-madec_ehmi_2019}, the 'visible percentage' is calculated in relation to how much of the vehicle is visible, not how much of that part of the car is visible on average. 

\subsubsection{Vehicle Kinematics as Indication (No eHMI)} 
Taking the sides of the vehicle as the 'display' of the eHMI, the vehicle kinematics are visible the most often in a vehicle \cite{troel-madec_ehmi_2019}. They are not visible when the observer is directly in front of the vehicle (\(P_{1_{No eHMI}} = 0\)), but they are visible from the front corners (\(P_{[2_{No eHMI}} = 1, P_{3_{No eHMI}} = 1\)), and when the vehicle is behind another vehicle (\(P_{{[9, 16]}_{No eHMI}} = 1\)). While not directly referenced in the study, one can safely assume the sides of the vehicle are visible when standing and observing directly at them (\(P_{4_{No eHMI}} = 1, P_{5_{No eHMI}} = 1\)).

\subsubsection{Front Braking Lights (FBL), Knight Rider Display (KRD), Grill Smile Display (BSD), Grill Text Display (BTD)}
Since all of these proposals use displays mounted on the front, they are all visible directly from the front (\(P_{1} = 1\)). According to \cite{troel-madec_ehmi_2019}, the front of the vehicle is also visible from the front corners of the vehicle (\(P_{[2} = 1, P_{3} = 1\)), but only when it doesn't have another vehicle in front of it.
}

%\begin{table}[ht]
\input{tables/results6}
%\end{table}

==> results/readability_results.tex <==

\subsection{Readability Scores}
While plenty of research has been conducted on the readability of screens under different lighting conditions, these studies mainly focus on mobile devices with lower luminance than the vehicle display used in \cite{ledsigncity_car_nodate} \cite{}
These results are reflected in \ref{tab:result7_table}. All proposals with a display can adjust their brightness based on weather and lighting conditions (\(R_{{1 to 3}_{KRD}} = 1, R_{{1 to 3}_{BSD}} = 1, R_{{1 to 3}_{BTD}} = 1\)).

Otherwise, there is no sufficiently empirical data to evaluate the visibility of the selected proposals in the specified conditions (\(R_{{1 to 40}_{No eHMI}} = 0, R_{{1 to 40}_{FBL}} = 0, R_{{4 to 40}_{KRD}} = 0, R_{{4 to 40}_{BSD}} = 0, R_{{4 to 40}_{BTD}} = 0\)).

\begin{table}[ht]
\input{tables/results7}
\end{table}

==> results/standardization_results.tex <==
\subsection{Standardization Scores}
Since each proposal may have multiple individual separate eHMIs to communicate information, this section evaluates each proposal independently. None of the proposals make use of sound, and for the purpose of this evaluation all proposals have their position on the vehicle specified.

\subsubsection{Vehicle Kinematics as Indication (No eHMI)} 
This proposal has only one element: The vehicle chassis that shows the kinematic motions of the vehicle as it comes to a stop.
\paragraph{Element 1: Vehicle Chassis} Since the kinematic motion of the vehicle is built into its primary functionality, standardization of it requires no additional work. As seen in Table \ref{tab:result1_table1}, most of the questions were not applicable to this proposal, except for two exceptions:
\begin{itemize}
    \item The proposal relies on kinematic motions to communicate a stopping action, and hence yielding intent. It does not have a kinematic way to indicate when it is not stopping beyond the absence of the stopping behavior, and the acceleration of the vehicle isn't accompanied by other motions to draw attention to it. This means \(Aks = 1\), which results in \(S_{23_{{No eHMI}_1}} = 1\). 
    \item Three  conditions may trigger a change in the stopping motion: Whether the vehicle is stopping or not (counted as one condition), the distance between the vehicle and it's stopping destination, and the deceleration rate of the vehicle. This results in \(S_{27_{{No eHMI}_1}} = 3\). 
\end{itemize}

\begin{table}[h]
\input{tables/results1_1}
\end{table}

\subsubsection{Front Braking Lights (FBL)} 
Made up of two lights, identical to each other, so they are counted as one eHMI.
\paragraph{Element 1: Lights} 
For the purposes of this evaluation, the lights were treated as "Pictograms". This proposal does not use frames, background, text or animations. It contains displays that can be turned off (\(S2 = 1\)); can be manufacturer to produce more than one color of light (\(S11 = 1\)); must decide when to turn on based on yielding decision and distance from the pedestrian (\(S12 = 2\)); and has two possible states for yielding and unyielding (\(S15 = 2 - 1\)). 

\begin{table}[h]
\input{tables/results1_2}
\end{table}

\subsubsection{Knight Rider Display (KRD)}
Made up of two elements: One display on the front bumper, and seven LED lights on the hood that light up in synchronicity with the bumper display.
\paragraph{Element 1: Display} 
For the purpose of this evaluation, the sweeping animation on the display is treated as a pictogram. It does not make use of text. It contains a display that can be turned off (\(S2 = 1\)); has a frame that can be made in more than one color (\(S4 = 1\)) and thickness (\(S5 = 1\)); has a background to the lights that can be made in more than one color (\(S7 = 1\)); may change its animation based on yielding decision and distance from the stopping position (\(S10 = 2\)); the display itself can be made in a variety of colors (\(S11 = 1\)); and has two possible states for yielding and unyielding (\(S15 = 2 - 1\)). 
Additionally, it features an intermittent animation (\(Arc = 1\)) that loops every 0.5 second (\(Ams = 500\))\cite{de_clercq_external_2019}.
\paragraph{Element 2: Lights} 
The group of lights on the hood do not make use of frames, text, or a background. They can be turned off (\(S2 = 1\)); can be manufactured in a variety of colors (\(S11 = 1\)); have two possible states for yielding and unyielding (\(S15 = 2 - 1\)); has the same animation timing as the main display (\(Arc = 1, Ams = 500\)). Its determining condition is whether the main display is in an animated or static state (\(S27 = 1\)).

\begin{table}[h]
\input{tables/results1_3}
\vspace{0.5cm}
\input{tables/results1_4}
\end{table}

\subsubsection{Bumper Smile Display (BSD)}
Made up of one element: A display on the front bumper that shows a grin when the vehicle is yielding, and maintains a straight line that simulates a neutral expression otherwise.
\paragraph{Element 1: Display}
The smile is a pictogram. The display does not make use of text. It can be turned off (\(S2 = 1\)); has a frame that can be made in more than one color (\(S4 = 1\)) and thickness (\(S5 = 1\)); has a background to the lights that can be made in more than one color (\(S7 = 1\)); may change its pictogram  based on yielding decision and distance from the stopping position (\(S10 = 2\)); the display itself can be made in a variety of colors (\(S11 = 1\)); and has two possible states for yielding and unyielding (\(S15 = 2 - 1\)). 

\begin{table}[h]
\input{tables/results1_5}
\end{table}

\subsubsection{Bumper Text Display (BTD)}
Made up of one element: A display on the front bumper that can show text indicating the intent of the vehicle.
\paragraph{Element 1: Display}
The display does not make use of pictograms. It can be turned off (\(S2 = 1\)); uses text that needs standardization of font, letter spacing, color, and size (\(S3 = 4\)); has a frame that can be made in more than one color (\(S4 = 1\)) and thickness (\(S5 = 1\)); has a background to the text that can be made in more than one color (\(S7 = 1\)); may change its text content based on yielding decision and distance from the stopping position (\(S16 = 2\)); the display itself can be made in a variety of colors (\(S17 = 1\)); and has two possible states for yielding and unyielding (\(S18 = 2 - 1\)). 


\begin{table}[h]
\input{tables/results1_6}
\end{table}

\subsubsection{Results}
Since vehicle kinematics, by definition, require no additional eHMI standardization, the standardization baseline value is calculated using Equation (\ref{BaselineCalculation:12}), where \({S_{count}} = 27\) and \({S_{P_{no eHMI}}} = 4\).
After adding up the penalties across all elements for each proposal using Equation (\ref{SPx:1}) and calculating the Standardization Score for each using Equation (\ref{S_S:2}), the results show Frontal Brake Lights and Bumper Smile Display as the easiest proposals to standardize after the vehicle kinematics, while the Knight Rider Display scores lowest due to its multiple non-identical eHMIs. 

\begin{table}[h]
\input{tables/results1_total}
\end{table}

==> tables/positioning_test_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[h]
\begin{adjustwidth}{-2cm}{-2cm}
\centering
\tiny
\begin{tabular}{|
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}l |cccccccccc|}
\hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{B7B7B7}} & \multicolumn{10}{c|}{\cellcolor[HTML]{CCCCCC}\begin{tabular}[c]{@{}c@{}}Is there a Grid Point in the part of the vehicle that was recorded an amount of times \\ equal or higher than 50\% of the highest value under these conditions?\end{tabular}} \\ \hline
\multicolumn{2}{|l|}{\cellcolor[HTML]{D9D9D9}Road occupied by vehicle...} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Left \\ Side\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Right\\ Side\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Left \\ Side\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Right \\ Side\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Right \\ Alleyway\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Left \\ Alleyway\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Either\\ Alleyway\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Left\\ Lane\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Left\\ Lane\end{tabular}} & \cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Left\\ Lane\end{tabular} \\ \hline
\multicolumn{2}{|l|}{\cellcolor[HTML]{D9D9D9}Place occupied by observer...} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Left\\ Sidewalk\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Left\\ Sidewalk\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Left\\ Sidewalk\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Left\\ Sidewalk\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Left\\ Sidewalk\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Left\\ Sidewalk\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Either\\ Lane\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Right\\ Lane\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Left\\ Lane\end{tabular}} & \cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}c@{}}Left\\ Lane\end{tabular} \\ \hline
\multicolumn{2}{|l|}{\cellcolor[HTML]{D9D9D9}\begin{tabular}[c]{@{}l@{}}Observer is looking towards \\ the vehicle's...\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}Front} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}Front} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}Back} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}Back} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}Front} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}Front} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}Front} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}Front} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}Front} & \cellcolor[HTML]{D9D9D9}Back \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & \begin{tabular}[c]{@{}l@{}}...anywhere on the \\ back bumper.\end{tabular} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & Yes \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & ...the back central light. & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & ...either of the back fenders. & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & \begin{tabular}[c]{@{}l@{}}...anywhere on the\\ back low reflector.\end{tabular} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & Yes \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & \begin{tabular}[c]{@{}l@{}}...the location of \\ the back plate.\end{tabular} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & Yes \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & \begin{tabular}[c]{@{}l@{}}...either of the back window \\ rails.\end{tabular} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & \begin{tabular}[c]{@{}l@{}}...anywhere on the back \\ window.\end{tabular} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & Yes \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & \begin{tabular}[c]{@{}l@{}}...anywhere on the back \\ window's lower frame.\end{tabular} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & Yes \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & \begin{tabular}[c]{@{}l@{}}...anywhere on the cowl\\ cover.\end{tabular} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & \begin{tabular}[c]{@{}l@{}}...anywhere on the front \\ bumper.\end{tabular} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & \begin{tabular}[c]{@{}l@{}}...anywhere on the front low \\ reflector.\end{tabular} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & \begin{tabular}[c]{@{}l@{}}...anywhere on \\ either of the front doors.\end{tabular} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & ...either of the front fenders. & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & \begin{tabular}[c]{@{}l@{}}...the location of the front\\ plate.\end{tabular} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & \begin{tabular}[c]{@{}l@{}}...either of the windshield\\ side rails.\end{tabular} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & ...either of the front wheels. & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & ...either of the front windows. & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & ...anywhere on the grill. & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & ...either headlight. & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & ...anywhere on the hood. & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & ...either of the back doors. & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & ...either of the rear wheels. & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & ...either of the rear windows. & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & ...either of the rocker panels. & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & ...roof. & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & ...either of the side mirrors. & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & \begin{tabular}[c]{@{}l@{}}...either of the side mirror's\\ front.\end{tabular} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & ...anywhere on the windshield. & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & ...either tail light. & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & No \\ \cline{2-12} 
\multicolumn{1}{|c|}{\multirow{-30}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}T\\ h\\ e\\ \\ e\\ H\\ M\\ I\\  \\ i\\ s\\  \\ p\\ o\\ s\\ i\\ t\\ i\\ o\\ n\\ e\\ d\\ .\\ .\\ .\end{tabular}}} & ...anywhere on the trunk. & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & Yes \\ \hline
\end{tabular}
\caption{Visibility of different external vehicle elements, based on their heatmap results.}
\label{tab:my-position_test_results}
\end{adjustwidth}
\end{table}

==> tables/results10.tex <==
%\section{Environmental Sustainability} 
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
%\begin{table}[ht]
\centering
\caption{Environmental Sustainability Questionnaire Results}
\label{tab:result10_table}
\begin{tabular}{|lccccc|}
\hline
\multicolumn{6}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{ENVIRONMENTAL SUSTAINABILITY RESULTS}} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{CCCCCC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{No eHMI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{FBL}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{KRD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{BSD}} & \cellcolor[HTML]{D9D9D9}\textbf{BTD} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \textbf{1} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES2}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES3}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{1}} & \textbf{1} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES4}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES5}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \textbf{1} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES6}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES7}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES8}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES9}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES10}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES11}} & \multicolumn{1}{c|}{\textbf{2.5}} & \multicolumn{1}{c|}{\textbf{2.5}} & \multicolumn{1}{c|}{\textbf{2.5}} & \multicolumn{1}{c|}{\textbf{2.5}} & \textbf{2.5} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES12}} & \multicolumn{1}{c|}{\textbf{2.5}} & \multicolumn{1}{c|}{\textbf{2.5}} & \multicolumn{1}{c|}{\textbf{2.5}} & \multicolumn{1}{c|}{\textbf{2.5}} & \textbf{2.5} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES13}} & \multicolumn{1}{c|}{\textbf{2.5}} & \multicolumn{1}{c|}{\textbf{2.5}} & \multicolumn{1}{c|}{\textbf{2.5}} & \multicolumn{1}{c|}{\textbf{2.5}} & \textbf{2.5} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES14}} & \multicolumn{1}{c|}{\textbf{2.5}} & \multicolumn{1}{c|}{\textbf{2.5}} & \multicolumn{1}{c|}{\textbf{2.5}} & \multicolumn{1}{c|}{\textbf{2.5}} & \textbf{2.5} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES15}} & \multicolumn{1}{c|}{\textbf{10}} & \multicolumn{1}{c|}{\textbf{10}} & \multicolumn{1}{c|}{\textbf{10}} & \multicolumn{1}{c|}{\textbf{10}} & \textbf{10} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES16}} & \multicolumn{1}{c|}{\textbf{10}} & \multicolumn{1}{c|}{\textbf{10}} & \multicolumn{1}{c|}{\textbf{10}} & \multicolumn{1}{c|}{\textbf{10}} & \textbf{10} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES17}} & \multicolumn{1}{c|}{\textbf{10}} & \multicolumn{1}{c|}{\textbf{10}} & \multicolumn{1}{c|}{\textbf{10}} & \multicolumn{1}{c|}{\textbf{10}} & \textbf{10} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES18}} & \multicolumn{1}{c|}{\textbf{10}} & \multicolumn{1}{c|}{\textbf{10}} & \multicolumn{1}{c|}{\textbf{10}} & \multicolumn{1}{c|}{\textbf{10}} & \textbf{10} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES19}} & \multicolumn{1}{c|}{\textbf{10}} & \multicolumn{1}{c|}{\textbf{10}} & \multicolumn{1}{c|}{\textbf{10}} & \multicolumn{1}{c|}{\textbf{10}} & \textbf{10} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{ES20}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{2.27}} & \multicolumn{1}{c|}{\textbf{143.82}} & \multicolumn{1}{c|}{\textbf{143.79}} & \textbf{143.79} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{CCCCCC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{No eHMI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{FBL}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{KRD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{BSD}} & \cellcolor[HTML]{CCCCCC}\textbf{BTD} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{Baseline}} & \multicolumn{5}{c|}{70.00} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{Average Emissions}} & \multicolumn{5}{c|}{1237.00} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{TOTAL}} & \multicolumn{1}{c|}{10.00} & \multicolumn{1}{c|}{9.27} & \multicolumn{1}{c|}{7.69} & \multicolumn{1}{c|}{7.84} & 7.84 \\ \hline
\end{tabular}
%\end{table}

==> tables/results1_1.tex <==
%\section{Standardization} 

%\begin{table}[ht]
\caption{Standardization Questionnaire Results - Vehicle Kinematics}
\label{tab:result1_table1}
\centering
\begin{tabular}{|lllrllllll|}
\hline
\rowcolor[HTML]{CCCCCC} 
\multicolumn{10}{|c|}{\cellcolor[HTML]{CCCCCC}\textbf{NO EHMI: ELEMENT 1 (VEHICLE CHASSIS)}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{S1}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S2}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S4}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S5}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S6}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S7}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S8}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S9}} & \textbf{S10} \\ \hline
\multicolumn{1}{|r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{S11}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S12}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S13}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S14}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S15}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S16}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S17}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S18}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S19}} & \textbf{S20} \\ \hline
\multicolumn{1}{|r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{S21}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S22}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S23}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S24}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S25}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S26}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S27}} & \multicolumn{3}{l|}{\cellcolor[HTML]{EFEFEF}} \\ \cline{1-7}
\multicolumn{1}{|r|}{\textbf{0}} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{3}} & \multicolumn{3}{l|}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}}} \\ \hline
\multicolumn{3}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{Penalty Total}} & \multicolumn{7}{r|}{4} \\ \hline
\end{tabular}
%\end{table}

==> tables/results1_2.tex <==
%\section{Standardization} 

%\begin{table}[ht]
\caption{Standardization Questionnaire Results - Frontal Braking Lights}
\label{tab:result1_table2}
\centering
\begin{tabular}{|lllrllllll|}
\hline
\rowcolor[HTML]{CCCCCC} 
\multicolumn{10}{|c|}{\cellcolor[HTML]{CCCCCC}\textbf{FRONT BRAKING LIGHTS: ELEMENT 1 (LIGHTS)}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{S1}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S2}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S4}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S5}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S6}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S7}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S8}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S9}} & \textbf{S10} \\ \hline
\multicolumn{1}{|r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{S11}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S12}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S13}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S14}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S15}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S16}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S17}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S18}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S19}} & \textbf{S20} \\ \hline
\multicolumn{1}{|r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{2}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{S21}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S22}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S23}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S24}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S25}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S26}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S27}} & \multicolumn{3}{l|}{\cellcolor[HTML]{EFEFEF}} \\ \cline{1-7}
\multicolumn{1}{|r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{3}{l|}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}}} \\ \hline
\multicolumn{3}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{Penalty Total}} & \multicolumn{7}{r|}{5} \\ \hline
\end{tabular}
%\end{table}

==> tables/results1_3.tex <==
%\section{Standardization} 

%\begin{table}[ht]
\caption{Standardization Questionnaire Results - Knight Rider Screen Display}
\label{tab:result1_table3}
\centering
\begin{tabular}{|lllrllllll|}
\hline
\rowcolor[HTML]{CCCCCC} 
\multicolumn{10}{|c|}{\cellcolor[HTML]{CCCCCC}\textbf{KNIGHT RIDER DISPLAY: ELEMENT 1 (DISPLAY)}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{S1}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S2}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S4}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S5}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S6}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S7}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S8}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S9}} & \textbf{S10} \\ \hline
\multicolumn{1}{|r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{2}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{S11}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S12}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S13}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S14}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S15}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S16}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S17}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S18}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S19}} & \textbf{S20} \\ \hline
\multicolumn{1}{|r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{S21}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S22}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S23}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S24}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S25}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S26}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S27}} & \multicolumn{3}{l|}{\cellcolor[HTML]{EFEFEF}} \\ \cline{1-7}
\multicolumn{1}{|r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{1.5}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{3}{l|}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}}} \\ \hline
\multicolumn{3}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{Penalty Total}} & \multicolumn{7}{r|}{9.5} \\ \hline
\end{tabular}
%\end{table}

==> tables/results1_4.tex <==
%\section{Standardization} 

%\begin{table}[ht]
\caption{Standardization Questionnaire Results - Knight Rider LED Lights}
\label{tab:result1_table4}
\centering
\begin{tabular}{|lllrllllll|}
\hline
\rowcolor[HTML]{CCCCCC} 
\multicolumn{10}{|c|}{\cellcolor[HTML]{CCCCCC}\textbf{KNIGHT RIDER DISPLAY: ELEMENT 2 (LIGHTS)}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{S1}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S2}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S4}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S5}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S6}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S7}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S8}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S9}} & \textbf{S10} \\ \hline
\multicolumn{1}{|r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{S11}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S12}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S13}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S14}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S15}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S16}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S17}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S18}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S19}} & \textbf{S20} \\ \hline
\multicolumn{1}{|r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{S21}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S22}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S23}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S24}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S25}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S26}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S27}} & \multicolumn{3}{l|}{\cellcolor[HTML]{EFEFEF}} \\ \cline{1-7}
\multicolumn{1}{|r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{1.5}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{3}{l|}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}}} \\ \hline
\multicolumn{3}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{Penalty Total}} & \multicolumn{7}{r|}{5.5} \\ \hline
\end{tabular}
%\end{table}

==> tables/results1_5.tex <==
%\section{Standardization} 

%\begin{table}[ht]
\caption{Standardization Questionnaire Results - Bumper Smile Display}
\label{tab:result1_table5}
\centering
\begin{tabular}{|lllrllllll|}
\hline
\rowcolor[HTML]{CCCCCC} 
\multicolumn{10}{|c|}{\cellcolor[HTML]{CCCCCC}\textbf{BUMPER SMILE DISPLAY: ELEMENT 1 (DISPLAY)}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{S1}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S2}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S4}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S5}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S6}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S7}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S8}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S9}} & \textbf{S10} \\ \hline
\multicolumn{1}{|r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{2}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{S11}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S12}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S13}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S14}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S15}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S16}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S17}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S18}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S19}} & \textbf{S20} \\ \hline
\multicolumn{1}{|r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{S21}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S22}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S23}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S24}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S25}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S26}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S27}} & \multicolumn{3}{l|}{\cellcolor[HTML]{EFEFEF}} \\ \cline{1-7}
\multicolumn{1}{|r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{3}{l|}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}}} \\ \hline
\multicolumn{3}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{Penalty Total}} & \multicolumn{7}{r|}{8} \\ \hline
\end{tabular}
%\end{table}

==> tables/results1_6.tex <==
%\section{Standardization} 

%\begin{table}[ht]
\caption{Standardization Questionnaire Results - Bumper Text Display}
\label{tab:result1_table6}
\centering
\begin{tabular}{|lllrllllll|}
\hline
\rowcolor[HTML]{CCCCCC} 
\multicolumn{10}{|c|}{\cellcolor[HTML]{CCCCCC}\textbf{BUMPER TEXT DISPLAY: ELEMENT 1 (DISPLAY)}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{S1}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S2}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S4}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S5}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S6}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S7}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S8}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S9}} & \textbf{S10} \\ \hline
\multicolumn{1}{|r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{4}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{S11}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S12}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S13}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S14}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S15}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S16}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S17}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S18}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S19}} & \textbf{S20} \\ \hline
\multicolumn{1}{|r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{2}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{S21}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S22}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S23}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S24}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S25}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S26}} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{S27}} & \multicolumn{3}{l|}{\cellcolor[HTML]{EFEFEF}} \\ \cline{1-7}
\multicolumn{1}{|r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{1}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{1}{r|}{\textbf{0}} & \multicolumn{3}{l|}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}}} \\ \hline
\multicolumn{3}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{Penalty Total}} & \multicolumn{7}{r|}{11} \\ \hline
\end{tabular}
%\end{table}

==> tables/results1_total.tex <==
%\section{Standardization} 

%\begin{table}[ht]
\caption{Standardization Questionnaire Results - Standardization Results}
\label{tab:result1_table_total}
\centering
\begin{tabular}{|lccccc|}
\hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{6}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{STANDARDIZATION RESULTS}} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{Baseline}} & \multicolumn{5}{c|}{31} \\ \hline
\rowcolor[HTML]{CCCCCC} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{No eHMI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{FBL}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{KRD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{BSD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{BTD}} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{Penalty Total}} & \multicolumn{1}{r|}{4.00} & \multicolumn{1}{r|}{5.00} & \multicolumn{1}{r|}{15.00} & \multicolumn{1}{r|}{8.00} & 11.00 \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{TOTAL}} & \multicolumn{1}{r|}{10.00} & \multicolumn{1}{r|}{9.63} & \multicolumn{1}{r|}{5.93} & \multicolumn{1}{r|}{8.52} & 7.41 \\ \hline
\end{tabular}
%\end{table}

==> tables/results2.tex <==
%\section{Cost Effectiveness} 
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
%\begin{table}[ht]
\caption{Cost Effectiveness Questionnaire Results}
\label{tab:result2_table}
\centering
\begin{tabular}{|lrrrrr|}
\hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{6}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{COST EFFECTIVENESS RESULTS}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{CCCCCC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{No eHMI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{FBL}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{KRD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{BSD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{BTD}} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CE1}} & \multicolumn{1}{r|}{\textbf{0.00}} & \multicolumn{1}{r|}{\textbf{39.68}} & \multicolumn{1}{r|}{\textbf{4608.03}} & \multicolumn{1}{r|}{\textbf{4606.90}} & \textbf{4606.90} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CE2}} & \multicolumn{1}{r|}{\textbf{0.00}} & \multicolumn{1}{r|}{\textbf{43.00}} & \multicolumn{1}{r|}{\textbf{1.13}} & \multicolumn{1}{r|}{\textbf{0.00}} & \textbf{0.00} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CE3}} & \multicolumn{1}{r|}{\textbf{0.00}} & \multicolumn{1}{r|}{\textbf{43.00}} & \multicolumn{1}{r|}{\textbf{1.13}} & \multicolumn{1}{r|}{\textbf{0.00}} & \textbf{0.00} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CE4}} & \multicolumn{1}{r|}{\textbf{0.00}} & \multicolumn{1}{r|}{\textbf{53.94}} & \multicolumn{1}{r|}{\textbf{2303.46}} & \multicolumn{1}{r|}{\textbf{2303.45}} & \textbf{2303.45} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CE5}} & \multicolumn{1}{r|}{\textbf{0.00}} & \multicolumn{1}{r|}{\textbf{53.94}} & \multicolumn{1}{r|}{\textbf{27.62}} & \multicolumn{1}{r|}{\textbf{27.59}} & \textbf{27.59} \\ \hline
\rowcolor[HTML]{CCCCCC} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{CCCCCC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{No eHMI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{FBL}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{KRD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{BSD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{BTD}} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{Baseline}} & \multicolumn{5}{c|}{48301.00} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{TOTAL}} & \multicolumn{1}{r|}{10.00} & \multicolumn{1}{r|}{9.95} & \multicolumn{1}{r|}{8.56} & \multicolumn{1}{r|}{8.56} & 8.56 \\ \hline
\end{tabular}
%\end{table}

==> tables/results2_1.tex <==
%\section{Standardization} 

%\begin{table}[ht]
\caption{Cost Effectiveness Questionnaire Results - No eHMI}
\label{tab:result2_table1}
\centering
%\begin{table}[]
\begin{tabular}{|
>{\columncolor[HTML]{D9D9D9}}l r|}
\hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{NO EHMI RESULTS}} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{\(CE1_{No eHMI}\)}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{\(CE2_{No eHMI}\)}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{\(CE3_{No eHMI}\)}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{\(CE4_{No eHMI}\)}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{\(CE5_{No eHMI}\)}} & \textbf{0} \\ \hline
\end{tabular}
%\end{table}
%\end{table}

==> tables/results2_2.tex <==
\caption{Cost Effectiveness Questionnaire Results - Tail Lights}
\label{tab:result2_table2}
\centering
\begin{tabular}{|
>{\columncolor[HTML]{D9D9D9}}l r|}
\hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{TAIL LIGHTS RESULTS}} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CE1\_BrakeLight}} & \textbf{39.68} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CE2\_BrakeLight}} & \textbf{43.00} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CE3\_BrakeLight}} & \textbf{43.00} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CE4\_BrakeLight}} & \textbf{53.94} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CE5\_BrakeLight}} & \textbf{53.94} \\ \hline
\end{tabular}

==> tables/results2_3.tex <==
\caption{Cost Effectiveness Questionnaire Results - LED Display}
\label{tab:result2_table3}
\centering
\begin{tabular}{|
>{\columncolor[HTML]{D9D9D9}}l r|}
\hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{LED DISPLAY RESULTS}} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{\(CE1_{LED Display}\)}} & \textbf{4606.9} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{\(CE2_{LED Display}\)}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{\(CE3_{LED Display}\)}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{\(CE4_{LED Display}\)}} & \textbf{2303.45} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{\(CE5_{LED Display}\)}} & \textbf{27.59} \\ \hline
\end{tabular}

==> tables/results2_4.tex <==
\caption{Cost Effectiveness Questionnaire Results - LED Light Array}
\label{tab:result2_table4}
\centering
\begin{tabular}{|
>{\columncolor[HTML]{D9D9D9}}l r|}
\hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{LED LIGHT ARRAY RESULTS}} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{\(CE1_{LED Light Array}\)}} & \textbf{1.13} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{\(CE2_{LED Light Array}\)}} & \textbf{1.13} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{\(CE3_{LED Light Array}\)}} & \textbf{1.13} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{\(CE4_{LED Light Array}\)}} & \textbf{0.01} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{\(CE5_{LED Light Array}\)}} & \textbf{0.03} \\ \hline
\end{tabular}

==> tables/results3_1.tex <==
%\section{Accessibility} 

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[p]
\caption{Accessibility Questionnaire Results - Question A1 through A35}
\label{tab:result3_table1}
\tiny
\centering
\begin{tabular}{|lccccc|l|lccccc|}
\cline{1-6} \cline{8-13}
\multicolumn{6}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{ACCESSIBILITY RESULTS}} &
   &
  \multicolumn{6}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{ACCESSIBILITY RESULTS}} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{No eHMI}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{FBL}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{KRD}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{GSD}} &
  \cellcolor[HTML]{D9D9D9}\textbf{GTD} &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{No eHMI}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{FBL}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{KRD}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{GSD}} &
  \cellcolor[HTML]{D9D9D9}\textbf{GTD} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A1}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{0} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A39}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{0} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A2}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A40}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{0} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A3}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{0} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A41}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{0} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A4}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{0} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A42}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A5}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{0} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A43}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A6}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A44}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A7}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A45}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A8}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A46}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A9}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{0} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A47}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A10}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{0} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A48}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A11}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{0} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A49}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{0} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A12}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{0} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A50}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A13}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{0} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A51}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A14}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{0} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A52}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A15}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A53}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A16}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A54}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{0} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A17}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A55}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{0} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A18}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A56}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{0} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A19}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A57}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{0} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A20}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A58}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{0} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A21}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A59}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A22}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A60}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A23}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A61}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A24}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A62}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A25}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A63}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A26}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A64}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A27}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A65}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A28}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A66}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A29}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A67}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A30}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A68}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A31}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A69}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A32}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A70}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A33}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A71}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A34}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A72}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A35}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{0} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}\textbf{A73}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \multicolumn{1}{c|}{\textbf{1}} &
  \textbf{1} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A36}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{0} &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{No eHMI}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{FBL}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{KRD}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{GSD}} &
  \cellcolor[HTML]{CCCCCC}\textbf{GTD} \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A37}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{0} &
   &
  \multicolumn{1}{l|}{\cellcolor[HTML]{B7B7B7}\textbf{TOTAL}} &
  \multicolumn{1}{c|}{3.56} &
  \multicolumn{1}{c|}{5.07} &
  \multicolumn{1}{c|}{4.66} &
  \multicolumn{1}{c|}{4.66} &
  6.85 \\ \cline{1-6} \cline{8-13} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A38}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \multicolumn{1}{c|}{\textbf{0}} &
  \textbf{0} &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} \\ \cline{1-6} \cline{8-13} 
\end{tabular}
\end{table}

==> tables/results3_2.tex <==
%\section{Accessibility} 

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
%\begin{table}[p]
%\caption{Accessibility Questionnaire Results - Question A36 through A73}
%\label{tab:result3_table2}
%\tiny
%\centering
%\begin{tabular}{|l|c|c|c|c|c|}
%\hline
%\cellcolor[HTML]{D9D9D9}\textbf{A36} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A37} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A38} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A39} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A40} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A41} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A42} & \textbf{1} & \textbf{1} & \textbf{0} & \textbf{1} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A43} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A44} & \textbf{0} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A45} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A46} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A47} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A48} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A49} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A50} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A51} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A52} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A53} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A54} & \textbf{1} & \textbf{1} & \textbf{0} & \textbf{0} & \textbf{0} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A55} & \textbf{1} & \textbf{1} & \textbf{0} & \textbf{0} & \textbf{0} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A56} & \textbf{1} & \textbf{1} & \textbf{0} & \textbf{0} & \textbf{0} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A57} & \textbf{1} & \textbf{1} & \textbf{0} & \textbf{0} & \textbf{0} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A58} & \textbf{1} & \textbf{1} & \textbf{0} & \textbf{0} & \textbf{0} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A59} & \textbf{0} & \textbf{1} & \textbf{0} & \textbf{0} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A60} & \textbf{0} & \textbf{1} & \textbf{0} & \textbf{0} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A61} & \textbf{0} & \textbf{1} & \textbf{0} & \textbf{0} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A62} & \textbf{0} & \textbf{1} & \textbf{0} & \textbf{0} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A63} & \textbf{0} & \textbf{1} & \textbf{0} & \textbf{0} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A64} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A65} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A66} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A67} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A68} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A69} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A70} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A71} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A72} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\ \hline
%\cellcolor[HTML]{D9D9D9}\textbf{A73} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\ \hline
% & \cellcolor[HTML]{CCCCCC}\textbf{No eHMI} & \cellcolor[HTML]{CCCCCC}\textbf{FBL} & \cellcolor[HTML]{CCCCCC}\textbf{KRD} & \cellcolor[HTML]{CCCCCC}\textbf{BSD} & \cellcolor[HTML]{CCCCCC}\textbf{BTD} \\ \hline
%\cellcolor[HTML]{B7B7B7}\textbf{TOTAL} & 3.56 & 5.07 & 4.52 & 4.66 & 6.85 \\ \hline
%\end{tabular}
%\end{table}

==> tables/results4.tex <==
%\section{Ease of Understanding} 
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}
\caption{Ease of Understanding Questionnaire Results}
\label{tab:result4_table}
%\tiny
\centering
\begin{tabular}{|lccccc|}
\hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{6}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{EASE OF UNDERSTANDING RESULTS}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{CCCCCC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{No eHMI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{FBL}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{KRD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{BSD}} & \textbf{BTD} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{EU1}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{EU2}} & \multicolumn{1}{c|}{\textbf{65}} & \multicolumn{1}{c|}{\textbf{74}} & \multicolumn{1}{c|}{\textbf{79}} & \multicolumn{1}{c|}{\textbf{74}} & \textbf{76} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{EU3}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{EU4}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{EU5}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{EU6}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{EU7}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{EU8}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\rowcolor[HTML]{CCCCCC} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{CCCCCC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{No eHMI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{FBL}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{KRD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{BSD}} & \textbf{BTD} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{TOTAL}} & \multicolumn{1}{c|}{0.81} & \multicolumn{1}{c|}{0.93} & \multicolumn{1}{c|}{0.99} & \multicolumn{1}{c|}{0.93} & 0.95 \\ \hline
\end{tabular}
\end{table}

==> tables/results5.tex <==
%\section{Constant Communication} 
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[ht]
\centering
\caption{Constant Communication Questionnaire Results}
\label{tab:result5_table}
\tiny
\begin{tabular}{|lccccc|}
\hline
\multicolumn{6}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{CONSTANT COMMUNICATION RESULTS}} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{CCCCCC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{No eHMI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{FBL}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{KRD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{BSD}} & \cellcolor[HTML]{D9D9D9}\textbf{BTD} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{1} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC2}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC3}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC4}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC5}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \textbf{1} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC6}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC7}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC8}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC9}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC10}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC11}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC12}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC13}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC14}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \textbf{1} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC15}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \textbf{1} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC16}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC17}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC18}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC19}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC20}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC21}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC22}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC22}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC24}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{CCCCCC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{No eHMI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{FBL}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{KRD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{BSD}} & \cellcolor[HTML]{CCCCCC}\textbf{BTD} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{TOTAL}} & \multicolumn{1}{c|}{0.83} & \multicolumn{1}{c|}{0.42} & \multicolumn{1}{c|}{1.25} & \multicolumn{1}{c|}{1.25} & 1.67 \\ \hline
\end{tabular}
\end{table}

==> tables/results6.tex <==
%\section{Positioning} 
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
[WIP UPDATE]
\begin{table}[ht]
\centering
\caption{Positioning Questionnaire Results}
\label{tab:result6_table}
\tiny
\begin{tabular}{|lccccc|}
\hline
\multicolumn{6}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{POSITIONING RESULTS}} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{CCCCCC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{No eHMI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{FBL}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{KRD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{BSD}} & \cellcolor[HTML]{D9D9D9}\textbf{BTD} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \textbf{1} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P2}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \textbf{1} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P3}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P4}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P5}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P6}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P7}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P8}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P9}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P10}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P11}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P12}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{2}} & \textbf{2} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P13}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P14}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P15}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P16}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{2}} & \textbf{2} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P17}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P18}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P19}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P20}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P21}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P22}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P23}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P24}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P25}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P26}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P27}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P28}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P29}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P30}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P31}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P32}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P33}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \textbf{1} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P34}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P35}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \textbf{1} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P36}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P37}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P38}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P39}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P40}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \textbf{1} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{CCCCCC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{No eHMI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{FBL}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{KRD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{BSD}} & \cellcolor[HTML]{CCCCCC}\textbf{BTD} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{TOTAL}} & \multicolumn{1}{c|}{10.00} & \multicolumn{1}{c|}{6.00} & \multicolumn{1}{c|}{6.00} & \multicolumn{1}{c|}{6.00} & 6.00 \\ \hline
\end{tabular}
\end{table}

==> tables/results7.tex <==
%\section{Readability} 
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[ht]
\centering
\caption{Readability Questionnaire Results}
\label{tab:result7_table}
\tiny
\begin{tabular}{|lccccc|}
\hline
\multicolumn{6}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{READABILITY RESULTS}} \\ \hline
\multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{No eHMI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{FBL}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{KRD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{BSD}} & \cellcolor[HTML]{D9D9D9}\textbf{BTD} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R1}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \textbf{1} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R2}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \textbf{1} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R3}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \textbf{1} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R4}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R5}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R6}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R7}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R8}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R9}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R10}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R11}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R12}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R13}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R14}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R15}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R16}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R17}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R18}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R19}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R20}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R21}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R22}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R23}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R24}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R25}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R26}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R27}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R28}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R29}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R30}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R31}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R32}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R33}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R34}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R35}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R36}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R37}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{No eHMI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{FBL}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{KRD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{BSD}} & \cellcolor[HTML]{CCCCCC}\textbf{BTD} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{TOTAL}} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0.81} & \multicolumn{1}{c|}{0.81} & 0.81 \\ \hline
\end{tabular}
\end{table}

==> tables/results8.tex <==
%\section{Color} 
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
%\begin{table}[ht]
\centering
\caption{Color Questionnaire Results - Vehicle Kinematics}
\label{tab:result8_table}
\begin{tabular}{|lccccc|}
\hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{6}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{COLOR RESULTS}} \\ \hline
\rowcolor[HTML]{D9D9D9} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{CCCCCC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{No eHMI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{FBL}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{KRD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{BSD}} & \textbf{BTD} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{C1}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \textbf{1} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{C2}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \textbf{1} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{C3}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \textbf{1} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{C4}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \textbf{1} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{C5}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{1}} & \textbf{1} \\ \hline
\rowcolor[HTML]{CCCCCC} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{CCCCCC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{No eHMI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{FBL}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{KRD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{BSD}} & \textbf{BTD} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{TOTAL}} & \multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{8} & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{10} & 10 \\ \hline
\end{tabular}
%\end{table}

==> tables/results9.tex <==
%\section{Lighting Adaptation} 
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
%\begin{table}[ht]
\centering
\caption{Lighting Adaptation Questionnaire Results}
\label{tab:result9_table}
\begin{tabular}{|lccccc|}
\hline
\multicolumn{6}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{LIGHTING ADAPTATION RESULTS}} \\ \hline
\multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{No eHMI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{FBL}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{KRD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{BSD}} & \cellcolor[HTML]{D9D9D9}\textbf{BTD} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{LA1}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{LA2}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{LA3}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{LA4}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{LA5}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{LA6}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{LA7}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{LA8}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{LA9}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{LA10}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{LA11}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{LA12}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \multicolumn{1}{c|}{\textbf{0}} & \textbf{0} \\ \hline
\multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{No eHMI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{FBL}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{KRD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{BSD}} & \cellcolor[HTML]{CCCCCC}\textbf{BTD} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{TOTAL}} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} & 0 \\ \hline
\end{tabular}
%\end{table}

==> tables/testresults.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
%\begin{table}[ht]
\centering
\caption{Evaluation Results}
\label{tab:finalresults_table}
\begin{tabular}{|
>{\columncolor[HTML]{D9D9D9}}l ccccc|}
\hline
\multicolumn{6}{|c|}{\cellcolor[HTML]{D9D9D9}\textbf{FINAL RESULTS}} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{No eHMI}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{FBL}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{KRD}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{BSD}} & \cellcolor[HTML]{D9D9D9}\textbf{BTD} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{S}} & \multicolumn{1}{c|}{10.00} & \multicolumn{1}{c|}{9.63} & \multicolumn{1}{c|}{5.93} & \multicolumn{1}{c|}{8.52} & 7.41 \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CE}} & \multicolumn{1}{c|}{10.00} & \multicolumn{1}{c|}{9.95} & \multicolumn{1}{c|}{8.56} & \multicolumn{1}{c|}{8.56} & 8.56 \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{A}} & \multicolumn{1}{c|}{3.56} & \multicolumn{1}{c|}{5.07} & \multicolumn{1}{c|}{4.66} & \multicolumn{1}{c|}{4.66} & 6.85 \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{EU}} & \multicolumn{1}{c|}{0.81} & \multicolumn{1}{c|}{0.93} & \multicolumn{1}{c|}{0.99} & \multicolumn{1}{c|}{0.93} & 0.95 \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{CC}} & \multicolumn{1}{c|}{0.83} & \multicolumn{1}{c|}{0.42} & \multicolumn{1}{c|}{1.25} & \multicolumn{1}{c|}{1.25} & 1.67 \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{P}} & \multicolumn{1}{c|}{10.00} & \multicolumn{1}{c|}{6.00} & \multicolumn{1}{c|}{6.00} & \multicolumn{1}{c|}{6.00} & 6.00 \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{D9D9D9}\textbf{R}} & \multicolumn{1}{c|}{0.00} & \multicolumn{1}{c|}{0.00} & \multicolumn{1}{c|}{0.81} & \multicolumn{1}{c|}{0.81} & 0.81 \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{TOTAL}} & \multicolumn{1}{c|}{\textbf{35.21}} & \multicolumn{1}{c|}{\textbf{31.86}} & \multicolumn{1}{c|}{\textbf{28.06}} & \multicolumn{1}{c|}{\textbf{30.59}} & \textbf{32.11} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{B7B7B7}\textbf{\%}} & \multicolumn{1}{c|}{\textbf{50.30\%}} & \multicolumn{1}{c|}{\textbf{45.71\%}} & \multicolumn{1}{c|}{\textbf{40.28\%}} & \multicolumn{1}{c|}{\textbf{43.89\%}} & \textbf{46.07\%} \\ \hline
\end{tabular}
%\end{table}
